Large Scale Model Predictive Control with Neural Networks and Primal Active Sets

This work presents an explicit-implicit procedure to compute a model predictive control (MPC) law with guarantees on recursive feasibility and asymptotic stability. The approach combines an offline-trained fully-connected neural network with an online primal active set solver. The neural network provides a control input initialization while the primal active set method ensures recursive feasibility and asymptotic stability. The neural network is trained with a primal-dual loss function, aiming to generate control sequences that are primal feasible and meet a desired level of suboptimality. Since the neural network alone does not guarantee constraint satisfaction, its output is used to warm start the primal active set method online. We demonstrate that this approach scales to large problems with thousands of optimization variables, which are challenging for current approaches. Our method achieves a 2x reduction in online inference time compared to the best method in a benchmark suite of different solver and initialization strategies.

==> tex/ActiveSet.tex <==
\section{Active Set}

Duality theory and the usage of the Lagrangian allows us to handle constraints during training by minimizing the difference in the values corresponding to the predicted primal variables and the optimal primal variables. However, the neural network $\phi(\vec{x};\vec{\theta})$ is an approximation to the optimal control law $\vec{\mu}^{*}(\vec{x})$, and due to a variety of variables, such as the the non-convexity of the optimization problem~\eqref{eq:least_squares_Lagrangian} and the finite size of the dataset, there is no guarantee that the resulting learned neural network approximation will output feasible $\vec{z}^{\phi}$ for all feasible $\vec{x}$. In addition, while we can compute an upper bound on the sub-optimality of a specific $\vec{z}^{\phi}$ for a given $\vec{x}$ by computing the duality gap, we cannot compute a global upper bound. As a result, a secondary step is required to guarantee feasibility, a global sub-optimality bound, and thus asymptotic stability of the proposed control law.

The secondary step that we use is the \textit{active set method}. Active set methods solve a sequence of equality-constrained quadratic subproblems. The goal of these methods is the predict the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*}, \vec{x})$ that are tight, or satisfied with equality, at the optimal solution. The reason why we utilize this method over an alternative method to solve for the quadratic program are that these methods are well suited to \textit{warm-starts}, where a good initial guess of $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*}, \vec{x})$ can speed up the optimization method. On the other hand, path-following methods such as interior point methods like Mehrotra's Predictor Correct, are not well suited for warm-starts, since the warm-start point can be far away from the path, and as a result, many iterates are needed to get the initial point back on the path. 

Most active set methods require an initial feasible point. They thus consist of two phases, a \textit{Phase 1} method that finds an initial feasible point, and a \textit{Phase 2} method that takes this initial feasible point and performs the active set method algorithm. Given a $\tilde{\vec{z}}$ that is not too infeasible, the work required by the \textit{Phase 1} will be reduced~\cite{wright1999numerical}. In addition, given a $\tilde{\vec{z}}$ that is close to $\vec{z}^{*}$, the work required by the \textit{Phase 2} method will also be reduced. Thus a good approximation by our trained neural network $\vec{\phi}(\vec{x};\vec{\theta})$ will reduce the work required by both the Phase 1 and Phase 2 portions of the Active Set algorithm.

\subsection{Phase 1}
Let $\vec{g}^{(i)}_{0,\textrm{eq}}$ and $\vec{h}^{(i)}_{0,\textrm{eq}}$ for $i \in \mathcal{E}$ represent the $i$-th row of $\mat{G}_{0,\textrm{eq}}$ and $\mat{E}_{0,\textrm{eq}}\vec{x}$ respectively. In addition, let  $\vec{g}^{(i)}_{0,\textrm{in}}$ and $\vec{h}^{(i)}_{0,\textrm{in}}$ for $i \in \mathcal{E}$ represent the $i$-th row of $\mat{G}_{0,\textrm{in}}$ and $\vec{w}_{0,\textrm{in}}$ respectively.  Given the neural network output $\vec{\phi}(\vec{x};\vec{\theta})$, the Phase 1 method corresponds to solving the following linear feasibility problem:

\small
\begin{equation}
\label{eq:linear_feasibility_problem}
\begin{aligned}
& \underset{(\vec{z}, \vec{y})}{\text{argmin}}  
& & \vec{e}^{T}\vec{y} \\
& \text{s.t.}
& & \vec{g}^{(i)}_{0,\textrm{eq}}\vec{z} + \vec{\gamma}^{(i)}y^{(i)} = \vec{h}^{(i)}_{0,\textrm{eq}}, \qquad i \in \mathcal{E}\\
& & & \vec{g}^{(i)}_{0,\textrm{in}}\vec{z} + \vec{\gamma}^{(i)}y^{(i)} \leq \vec{h}^{(i)}_{0,\textrm{in}}, \qquad i \in \mathcal{I}\\
& & & \vec{y} \geq 0
\end{aligned}
\end{equation}
\normalsize

where $e = (1, \dots, 1)^{T}$, $\gamma^{(i)} = -\textrm{sign}(\vec{g}^{(i)}_{0,\textrm{eq}}\vec{\tilde{z}} - \vec{h}^{(i)}_{0,\textrm{eq}})$ for $i \in \mathcal{E}$, and $\gamma^{(i)} = -1$ for $i \in \mathcal{I}$. A feasible initial point for this problem is $\vec{z} = \vec{\tilde{z}}$, $y^{(i)} = |\vec{g}^{(i)}_{0,\textrm{eq}}\vec{\tilde{z}} - h^{(i)}_{0,\textrm{eq}}|$ for $i \in \mathcal{E}$, and $y^{(i)} = \max(\vec{g}^{(i)}_{0,\textrm{in}}\vec{z} + \vec{\gamma}^{(i)}y^{(i)} - \vec{h}^{(i)}_{0,\textrm{in}}, 0)$ for $i \in \mathcal{I}$. If $\vec{\tilde{z}}$ is feasible, then $(\vec{\tilde{z}}, \vec{0})$ is optimal for Problem~\eqref{eq:linear_feasibility_problem}. In addition, if Problem~\eqref{eq:decoupled_batch_problem} has a feasible solution, then the optimal objective function for Problem~\eqref{eq:linear_feasibility_problem} is $0$, and any solution yields a feasible point for Problem~\eqref{eq:decoupled_batch_problem}. 

\subsection{Phase 2}

Let $\vec{g}^{(i)}$ index the rows of both $\vec{g}^{(i)}_{0,\textrm{eq}}$, $\vec{g}^{(i)}_{0,\textrm{in}}$, and $\vec{h}^{(i)}$ index both $\vec{h}^{(i)}_{0,\textrm{in}}$ and $\vec{h}^{(i)}_{0,\textrm{eq}}$. If we know the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*},\vec{x})$, then we can solve the following equality constrained sub-problem:

\small
\begin{equation}
\label{eq:optimal_active_set_subproblem}
\begin{aligned}
& \underset{\vec{z}}{\text{argmin}}  
& & \vec{z}^{T}\mat{H}\vec{z} \\
& \text{s.t.}
& & \vec{g}^{(i)}\vec{z} = \vec{h}^{(i)}, \qquad i \in \mathcal{W}_{\mathcal{A}}(\vec{z}^{*},\vec{x})\\
\end{aligned}
\end{equation}
\normalsize
However, we do not necessarily know the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*},\vec{x})$ beforehand, but instead can get a good guess from the neural network output $\vec{z}^{\phi}$.

The Phase 2 method consists of starting with an initial feasible point $\vec{z}_{0}$ generated by the Phase 1 method, and computing an initial working set $\mathcal{W}_{0}$ containing a linearly independent subset of the active constraints at $\vec{z}_{0}$. It then iteratively computes a step direction $\vec{p}_{k}$ and updates $\mathcal{W}_{k}$ by either adding or removing constraints.

The step direction $\vec{p}_{k}$ is computed as follows. Define $\vec{p} = \vec{z} - \vec{z}_{k}$, and $\vec{g}_{k} = \mat{H}\vec{z}_{k}$. By substituting into the objective function of Problem~\eqref{eq:decoupled_batch_problem} and dropping the constant $\vec{x}^{T}\mat{Q}\vec{x}$ term, we get that 

\begin{equation}
\label{eq:active_step_step_objective}
\begin{aligned}
J_{0}(\vec{x},\vec{z}) &= \vec{z}^{T}\mat{H}\vec{z} \\
&= (\vec{z}_{k} + \vec{p})^{T}\mat{H}(\vec{z}_{k}+\vec{p}) \\
&= \vec{z}_{k}^{T}\mat{H}\vec{z}_{k} + 2\vec{z}_{k}^{T}\mat{H}\vec{p} + \vec{p}^{T}\mat{H}\vec{p} \\ 
&= \vec{p}^{T}\mat{H}\vec{p} + 2\vec{\eta}_{k}^{T}\vec{p} + c
\end{aligned}
\end{equation}
where $\eta_{k} = \mat{H}\vec{z}_{k}$, and $c = \vec{z}_{k}^{T}\mat{H}\vec{z}_{k}$ is a constant that does not depend on $p$. Thus by setting the constraints in $\mathcal{W}_{k}$ to equality and temporarily ignoring all other constraints, we can solve the equality-constrained sub-problem:

\small
\begin{equation}
\label{eq:active_set_subproblem}
\begin{aligned}
& \underset{\vec{p}}{\text{argmin}}  
& & \vec{p}^{T}\mat{H}\vec{p} + 2\vec{\eta}_{k}^{T}\vec{p} \\
& \text{s.t.}
& & \vec{g}^{(i)}\vec{p} = 0, \qquad i \in \mathcal{W}_{k}\\
\end{aligned}
\end{equation}
\normalsize

of which the solution is denoted as $\vec{p}_{k}$. Since $\vec{g}^{(i)}\vec{p}=0$, for each constraint $i \in \mathcal{W}_{k}$, it follows that if the constraint $\vec{g}^{(i)}\vec{z}_{k} = \vec{h}^{(i)}$ were satisfied at iteration $k$, then the constraint will also be satisfied at iteration $k+1$. If the optimal $\vec{p}_{k}$ is non-zero, we have to decide a step length $\alpha_{k}$ so that $\vec{z}_{k} + \alpha_{k} \vec{p}_{k}$ is still feasible for all constraints. We only have to worry about the constraints where $\vec{g}^{(i)}\vec{p}_{k} > 0$, thus we compute a step-length 

\begin{equation}
\label{eq:step_length}
\alpha_{k} = \min \left(1, \min_{i \neq \mathcal{W}_{k}, \vec{g}^{(i)}\vec{p}_{k}>0}\frac{h^{(i)}-\vec{g}^{(i)}\vec{z}_{k}}{\vec{g}^{(i)}\vec{p}_{k}} \right)
\end{equation}

and set $\vec{z}_{k+1} = \vec{z}_{k} + \alpha_{k}\vec{p}_{k}$. If $\alpha_{k} < 1$, then the the step along $\vec{p}_{k}$ was blocked by some constraint, and that constraint is added to $\mathcal{W}_{k}$ create a new working set $\mathcal{W}_{k+1}$.

These iterations are continued until a point $\hat{\vec{z}}$ is reached that minimizes the quadratic objective over the current working set $\mathcal{W}_{k}$. This can be identified because the solution to Problem~\eqref{eq:active_set_subproblem} will have a solution $\vec{p} = 0$. When this occurs, we inspect the Lagrange multipliers $\lambda_{i}$ corresponding to the inequality constraints in our current working set $\mathcal{W}_{k}$, that is $i \in \mathcal{W}_{k} \cap \mathcal{I}$. If all of the $\lambda_{i}$ are non-negative, then the $\vec{z}_{k}$ is a local optimizer, and thus a global optimizer.

If not, then we find the constraint $i$ with the most negative $\lambda_{i}$ and drop it from the working set $\mathcal{W}$ to get a new working set $\mathcal{W}_{k+1}$ and continue iterating.

Continuing in this fashion will eventually converge to the optimal solution $\vec{z}^{*}$ in a finite number of steps~\cite{wright1999numerical}. However, we usually will only care to reach a pre-specified $\epsilon$ level of sub-optimality and can terminate early. We can upper bound the sub-optimality of a feasible iterate $\vec{z}_{k}$ by computing the duality gap at each iteration, and terminating early once it is below $\epsilon$. See Alg~\eqref{alg:proposed_control_law}

\begin{algorithm}[t]
	\caption{Proposed Control Law}
	\label{alg:proposed_control_law}
	\begin{algorithmic}[1]
		\Procedure{Sub-Optimal Control Law}{$\vec{\theta}$, $\vec{x}$, $\epsilon$}
		\State $\tilde{\vec{z}} = \phi(\vec{x},\vec{\theta})$ \Comment{Call Neural Network}
		\State Compute feasible $\vec{z}_{0}$ from $\tilde{\vec{z}}$ by solving Eqn~\eqref{eq:linear_feasibility_problem}
		\State Set $\mathcal{W}_{0}$ to be a subset of active constraints at $vec{z}_{0}$
		\For{k=0,1,2,\dots}
			\State Solve Eqn.~\eqref{eq:active_set_subproblem} to find $\vec{p}_{k}$
			\If{$\vec{p}_{k} = 0$}
				\State Compute Lagrange multiplier $\hat{\lambda}_{i}$ and $\hat{\nu}_{i}$
				\If{$\hat{\lambda}_{i} \geq 0$ for $i \in \mathcal{W}_{k} \cap \mathcal{I}$}
					\State \Return{$\vec{z}_{k}$}
				\Else 
					\State Set $j = \argmin_{j \in \mathcal{W}_{k} \cap \mathcal{I}} \hat{\lambda_{i}}$
					\State $\vec{z}_{k+1} = \vec{z}_{k}$; $\mathcal{W}_{k+1} = \mathcal{W}_{k} \setminus \{j\}$
				\EndIf
			\Else{~($\vec{p}_{k} \neq 0$)}
				\State Compute $\alpha_{k}$ from Eqn.~\eqref{eq:step_length}
				\State $\vec{z}_{k+1} = \vec{z}_{k} + \alpha_{k}\vec{p}_{k}$
				\If{There are blocking constraints}
					\State Add blocking constraint to $\mathcal{W}_{k}$ to get $\mathcal{W}_{k+1}$
				\Else
					\State $\mathcal{W}_{k+1} = \mathcal{W}_{k}$
				\EndIf
			\EndIf
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}







==> tex/Analysis.tex <==
\section{Receding Horizon Controller Analysis}

\textcolor{red}{(Put in algorithm describing RHC)}
We implement our open loop mapping $\pi$ as a receding horizon controller (RHC). 



\begin{defn}(Control Invariant Set)
A set $\mathcal{C} \in \mathcal{X}$ is a control invariant set for system~\eqref{eq:system} subject to constraints~\eqref{eq:constraints} if
\begin{equation*}
\vec{x}(t) \in \mathcal{C} \implies ~\exists~\vec{u}(t) \in \mathcal{U} \textrm{ such that } \mat{A}\vec{x}(t) + \mat{B}\vec{u}(t) \in \mathcal{C}
\end{equation*}
\end{defn}

In the double integrator example, the Maximal LQR Invariant Set $\mathcal{O}_{\infty}^{LQR}$ is a control invariant set since $\vec{x}(t) \in \mathcal{O}_{\infty}^{LQR}$, and $\vec{u} = -\mat{K} \vec{x}(t)$ satisfies $\mat{A}\vec{x}(t) + \mat{B}\vec{u}(t) \in \mathcal{O}_{\infty}^{LQR}$. As mentioned previously, control invariant sets are usually computed by starting with a control invariant set and performing reachability analysis. A trivial control invariant set is the origin~\cite{borrelli2017predictive}.

\begin{defn}(Control Lyapunov Function)
A function $p: \mathbb{R}^{n} \rightarrow \mathbb{R}$ that is continuously differentiable, positive definite, and has the property
\begin{equation*}
\begin{aligned}
\min_{\vec{u} \in \mathcal{U}, \mat{A}\vec{x} + \mat{B}\vec{u} \in \mathcal{X}_{f}}(-p(\vec{x}) + q(\vec{x},\vec{u}) + p(\mat{A}\vec{x} + \mat{B}\vec{u})) &\leq 0, \\
&\forall~\vec{x} \in \mathcal{X}_{f}
\end{aligned}
\end{equation*}
where $q(\vec{x},\vec{u}) = \vec{x}^{T}\mat{M}\vec{x} + \vec{u}^{T}\mat{R}\vec{u}$, is called a control Lyapunov function.
\end{defn}

The choice of terminal cost $\vec{x}_{N}^{T}\mat{P}_{\infty}\vec{x}_{N}$ satisfies the conditions of a control Lyapunov function.

\subsection{Recursive Feasibility and Asymptotic Stability of Optimal Mapping}
Suppose we compute the optimal open loop mapping $\pi^{*}$ where $\vec{z}^{*} = \pi^{*}(\vec{x}(t))~\forall~\vec{x}(t) \in \mathcal{X}_{0}$. The following theorem establishes conditions on the terminal constraint region $\mathcal{X}_{f}$ and the terminal cost penalty $\vec{x}^{T}_{N}\mat{P}\vec{x}_{N}$ that guarantee recursive feasibility and asymptotic stability of the corresponding optimal RHC $\pi_{0}^{*}$.

\begin{thm}(Recursive Feasibility and Asymptotic Stability of the optimal RHC)
\label{thm:optimal_rf_as}
Choose $\mathcal{X}_{f}$ to be a control invariant set, and choose $\mat{P}$ such that $\vec{x}_{N}^{T}\mat{P}\vec{x}_{N}$ is a control Lyapunov function, then the optimal RHC $\pi_{0}^{*}$ is recursively feasible and asymptotically stable with domain of attraction $\mathcal{X}_{0}$ for system~\eqref{eq:system} subject to constraints~\eqref{eq:constraints}.
\end{thm}
\begin{pf}
See ~\cite[Thm 12.1]{borrelli2017predictive} for recursive feasibility and ~\cite[Thm 12.2]{borrelli2017predictive} for asymptotic stability.
\end{pf}

For the double integrator example, since our choice of the terminal region $\mathcal{O}_{\infty}^{LQR}$ and cost penalty $\mat{P}_{\infty}$ satisfy the definitions of a control invariant set and control Lyapunov Function, due to Thm~\ref{thm:optimal_rf_as},  the optimal RHC $\pi_{0}^{*}$ is recursively feasible and asymptotically stable.

\subsection{Recursive Feasibility and Asymptotic Feasibility of Approximate Mapping}

Rather than computing the optimal $\pi^{*}$, it may be preferable to compute an approximate sub-optimal open loop mapping $\pi^{A}$ due to computational constraints. We need to establish the conditions where the corresponding  approximate RHC $\pi_{0}^{A}$ have the recursive feasibility and asymptotic stability properties. The following theorem establishes the conditions that guarantee these properties:


\begin{thm}(Recursive Feasibility and Asymptotic Stability of an Approximate RHC)
	\label{thm:approximate_RHC_stability}
	Choose $\mathcal{X}_{f}$ to be a control invariant set, and choose $\mat{P}$ such that $\vec{x}_{N}^{T}\mat{P}\vec{x}_{N}$ is a control Lyapunov function. Suppose for an approximate feasible parametric solution $\pi$, there exists a function $\gamma(\vec{x})$ where $\mathbf{dom}(\gamma) = \mathcal{X}_{0}$
	\begin{equation*}
	\begin{aligned}
	&\sigma(\pi(\vec{x}); \vec{x}) \leq \gamma(\vec{x}),~ \forall~\vec{x} \in \mathcal{X}_{0}, \\
	&\gamma(\vec{x}) \geq 0,\\
	&\gamma(\vec{x}) - q(\vec{x},\vec{0}) \leq 0,
	\end{aligned}
	\end{equation*}  
	then the corresponding approximate RHC $\pi_{0}$ is recursively feasible and asymptotically stable with domain of attraction $\mathcal{X}_{0}$ for system~\eqref{eq:system} subject to constraints~\eqref{eq:constraints}. In addition, we call the open loop mapping $\pi$ a $\gamma$-suboptimal open loop mapping.
\end{thm}
\begin{pf}
	A similar argument as for the optimal case proves recursive feasibility. See ~\cite[Thm 13.1]{borrelli2017predictive} for asymptotic stability.
\end{pf}



By choosing control invariant $\mathcal{X}_{f}$, recursive feasibility holds for the approximate RHC. In addition, with the proper choice of $\mat{P}$, if we can provide an upper bound the sub-optimality level of $\pi$ by the portion of first stage cost $\vec{x}^{T}\mat{M}\vec{x}~\forall \vec{x} \in \mathcal{X}_{0}$ globally, then we can guarantee asymptotic stability of the approximate RHC.





==> tex/Discussion.tex <==
\section{Discussion and Analysis}

\subsection{Motivation for combining explicit and implicit MPC}
\label{sec:providing_guarantees}

It is clear that the role of the active set component is to achieve primal feasibility and pre-determined sub-optimality of the predicted primal variables, which in turn guarantee recursive feasibility and asymptotic stability of the $\pi_{0}^{A}$. The proposed control law thus provides \textit{guarantees by construction}.

An alternative approach is to provide statistical \textit{guarantees by verification}. For example, if one has the ability to generate i.i.d data inputs, one can construct a held-out validation set of arbitrary size. This alternative control law training algorithm increases the data set size and training time until a desired level of performance is achieved on the held-out validation set. Concentration inequality techniques such as Hoeffding's Inequality can then be applied to achieve statistical guarantees of recursive feasibility and asymptotic stability~\cite{Hertneck2018}. 

However, as noted in previous work~\cite{Hertneck2018}, in practice, it can be challenging to train a network to the necessary accuracy. Our own experiences mirror these observations. Anecdotally, in other fields such as computer vision, more and more complicated architectures and algorithms are being used to obtain smaller and smaller gains in performance on tests sets. This trend indicates that these neural networks tend to have diminishing marginal gains and are not able to achieve arbitrarily low validation errors.

These challenges can occur for a variety of reasons, such as not choosing a neural network with large enough capacity, the inability to train the network to a global optima, and the inability to generalize well. In addition, the training process for neural networks largely remains heuristic-based, with a lot of tunable hyperparameters such as learning rate, batch size, learning algorithms, data set size, training time etc. In addition, there typically is not a clear relation between these factors and the resulting neural network performance. For example, intuition would say that longer training times would improve validation accuracy, however a large family of algorithms use the idea of \textit{early stopping} as a regularization method to improve generalization~\cite{Goodfellow-et-al-2016}.

Due to these issues, an algorithm which requires the network to achieve necessary accuracy on the validation may not necessarily terminate. In addition, even if it does achieve the necessary accuracy, the resulting size of training time for such a network may be impractically large. As a result, such an approach, while appealing theoretically, may not practical for large problem sizes. 

Combining the strengths of explicit and implicit MPC methods has been explored in previous work~\cite{zeilinger2011real}. The purpose of introducing the online optimization component was to reduce the computational complexity of computing and calling the approximate explicit MPC control law. Similarly, by introducing this online active set component, we can potentially reduce the complexity of our neural network architecture. However, more importantly, the combination provides \textit{guarantees by construction}, and prevents many of the difficulties associated with an approach that relies solely on statistical guarantees using a validation set. The proposed algorithm mimics a design philosophy similar to that in~\cite{Chen2018ApproximatingEM} of using traditional control theoretic techniques to provide the framework to guarantee desirable properties, while using deep learning to optimize performance within that framework.

At the same time, however, it is still beneficial to integrate statistical analysis on a validation set to analyze the learned control law. Specifically, the following section will detail how we can use these techniques to provide a statistical confidence bound on the maximum number of active set iterations needed by our proposed control law. By comparing the statistics on the number of active set iterations required by our proposed control law with to those required if we were to just perform the active set method from a random initialization, we can quantify the benefit of using the neural network, as well as determine which regions in the state space it does not perform well. If, for example, we find that no active set iterations are required, than our analysis becomes a statistical \textit{guarantee by verification}. 

%However, the motivation for combining the two methods in our proposed approach differs than in these previous. Or motivation is to use the active set method primarily as a method to provide a guarantee, but in practice the quality of the neural network approximation is usually good enough such that very few iterations of the active set method are needed. In addition, as noted in~\cite{wang2010fast}, solving the optimization problem~\eqref{eq:decoupled_batch_problem} to the optimum is not necessary to achieve very good control law performance, and good control law results are obtainable even when primal feasibility is not achieved. As a result, using the neural network component of the control law already achieves good control performance, as demonstrated in our results section, highlighting the role of the active set method mostly as an analytical tool. 

%On the other hand, the previous works that combine explicit and implicit MPC methods, such as~\cite{zeilinger2011real}, use the active set method to decrease the computational burden of the approximate explicit parametric solution and improve the performance of the resulting closed-loop controller. In these methods, in order to maintain analytical tractability, the form of the explicit control law is designed to be analytically tractable, for example being able to prove primal feasibility by construction. As a result analytical tractability, the method does not scale well to large problem sizes, and the role of the active set method is to both increase performance of simpler approximate explicit control law.



\subsection{Bounds on Number Active Set Iterations}
\label{sec:statstical_verification}

The main boon to our problem is the ability to generate new i.i.d. data at will. As a result, we can provide strong results using traditional statistical estimation techniques that rely on these i.i.d. assumptions and apply in the limit of large numbers. Examples of such theorems are the Central Limit Theorem for sums and averages, and the Fisher-Tippett-Gnedenko Theorem for maximum~\cite{coles2001introduction}. While we can apply these theorems to evaluate a trained control law on a validation set, the argument made in the previous section Sec~\ref{sec:providing_guarantees} is to move away from the paradigm of iterating between training and verification, because the training step for the neural networks is currently not well-controlled in the sense that there are not clear parameters to tune to reach the necessary levels of performance.

Besides the standard bounds on the error computed by~\cite{Hertneck2018}, another desirable property to model is the number of iterations required by the active set component of our proposed control law. We can use statistical techniques to estimate these properties by the use of a validation set. For example, we can estimate the mean number of iterations required by taking the empirical mean on our validation set and using the Central Limit Theorem.

We would also like to know the \textit{maximum} number of iterations we should expect to require by using our control law. We know that this number is finite, since the active set method terminates in finite time. By estimating this maximum, we can quantitatively compare the effectiveness of combining the neural network with the active set method versus a purely implicit MPC approach of using only the active set method.

To estimate this maximum, we can use standard techniques from Extreme Value Theory (EVT), which model the maximum of i.i.d random variables using a Generalized Extreme Value (GEV) distribution~\cite{coles2001introduction}, and use maximum likelihood estimation (MLE) to choose the best parameters within the GEV distribution. Given this model, we can then estimate probabilities that the maximum number of iterations required is a specific quantity.






\subsection{Role of Neural Network}

Our neural network approximated the optimal parametric solution $\pi^{*}$. However, there are a variety of other functions the neural network can approximate. For example, the neural network can be used to output the Q-value of a state, action pair $\vec{\phi}(\vec{x},\vec{u};\vec{\theta}):\mathbb{R}^{n} \times \mathbb{R}^{m} \rightarrow \mathbb{R}$. This is the approach used by deep reinforcement learning methods such as Deep Q-Networks~\cite{mnih2015human}. However, Q-learning methods are difficult to apply to continuous action problems~\cite{gu2016continuous} due to the need to perform an $\argmin$ operation over a potentially non-convex function to derive the policy.

An alternative is rather than having the neural network output the entire sequence of predicted states and control inputs, it can map the state to $\pi_{0}^{A}$, outputting only the first control input. This role is similar to the approach used by many deep reinforcement learning methods based on policy gradients~\cite{mnih2016asynchronous}. However, the drawback of this approach is that if the neural network outputs an infeasible control input, it is challenging to correct it in a way that guarantees feasibility or stability. In addition, it is not possible to compute the sub-optimality measures using only the first control input.

The drawback of such our approach is that the output size of the network is much larger. However, the benefit is that by outputting all of the primal variables, it is possible to use the network output as an initial guess $\vec{z}^{init}$ to for the active set component.

%It is not clear how the size of the neural network is dependent on the network output size, and this issue is not investigated in this work. However, 

The proposed control framework is flexible to various online inference demands. For example, in applications where inference speed is critical, one option is to utilize two networks $\phi_{0}(\vec{x};\vec{\theta}): \mathbb{R}^{n} \rightarrow \mathbb{R}^{m}$ and $\phi_{1}(\vec{x};\vec{\theta}): \mathbb{R}^{n} \rightarrow \mathbb{R}^{(N\cdot n+ (N-1)\cdot m)}$, where $\phi_{0}$ maps the state to the first control input, and $\phi_{1}$ maps the state to the remaining decision variables in $\vec{z}$. With this approach, $\phi_{0}$, can be called at a high frequency as fast as possible (utilizing a simple heuristic projection if necessary), while $\phi_{1}$, and the active set method, can be called at a slower rate to provide guarantees of recursive feasibility and asymptotic stability. In addition, by analyzing the control law at different parts of the state space $\mathcal{X}_{0}$ using statistical techniques similar to those Sec.~\ref{sec:statstical_verification}, the user can pre-determine at which regions it is necessary to call $\phi_{1}$.


\subsection{Choice of Training Algorithm}
Our proposed algorithm uses the supervised learning algorithm. Another common training paradigm is called reinforcement learning (RL), where a learning agent discovers optimal behavior through interaction with the environment. Deep RL has gained a lot of popularity recently, where methods such as policy gradient algorithms~\cite{schulman2015trust} are used to optimize a neural network approximating the first control input $\pi_{0}^{A}$. Algorithms motivated by RL have been applied to MPC problems in~\cite{Chen2018ApproximatingEM}.

RL methods work well when there are many unknowns in the problem, and optimal labels are not easily computed to generate the dataset. For example, these methods usually assume nothing about the system dynamics, and the costs may also be unknown and have to be discovered by interactively probing the system. As a result of these difficulties, the RL paradigm is a more general framework than SL, but comes at the cost of additional difficulties, such as the exploration/exploitation dilemma not encountered in the SL framework~\cite{kober2013reinforcement}. Deep RL methods have empirically been found to require very high sample complexity, or training times~\cite{gu2016q}. 

In our problem setup, we have the ability to independently sample training examples $\vec{x}(t) \in \mathcal{X}_{0}$. In addition, convex QP solvers can efficiently return the optimal primal and dual variables of optimization problem~\eqref{eq:decoupled_batch_problem}. As a result, our problem formulation fits the assumptions and practical requirements of an SL paradigm, and is the learning framework of choice to train the neural network.

\subsection{Choice of Loss Function}
\label{sec:loss_functions}
In our supervised learning framework, we minimized the $\ell_{2}$ error between the network Lagrangian value and the optimal Lagrangian value. The choice of loss function can have a large effect on the performance of the resultant neural network. Recall that our neural network will represent an approximate open-loop parametric solution $\pi^{A}(\vec{x}) = \phi(\vec{x};\vec{\theta})$.

\textbf{Sub-optimality Loss}: The ideal loss function we would like to optimize for is the sub-optimality level of the approximate open-loop parametric solution, since we need to bound this sub-optimality level to apply Theorem~\ref{thm:approximate_RHC_stability}.:

\begin{equation}
\label{eq:true_metric}
\sum_{i=1}^{N_{B}} \left[ \sigma(\phi(\vec{x}_{i};\vec{\theta}),\vec{x}_{i}) \right] ^{2}
\end{equation}

This loss function would be easy to utilize if the neural network was approximating the value $J_{0}(\vec{x_{i}})$ for a given $\vec{x}_{i})$. However, since the neural network is approximating the parametric solution, this approach will not work since minimizing such a loss will not be able to handle the constraints in Problem~\eqref{eq:decoupled_batch_problem}. 

When the constraints are enforced,  $J_{0}(\vec{x}_{i},\phi(\vec{x}_{i};\vec{\theta})) \geq J_{0}^{*}(\vec{x}_{i})$ by definition of the solution of~\eqref{eq:decoupled_batch_problem}. In addition, if $J_{0}(\vec{x}_{i},\phi(\vec{x}_{i};\vec{\theta})) = J_{0}^{*}(\vec{x}_{i})$, then $\vec{z}^{*}(\vec{x}) = \phi(\vec{x}_{i};\vec{\theta})$ due to uniqueness since $\mat{H}$ is strictly positive definite.

However, when constraint satisfaction is not explicitly handled during training, which is the case when the ideal loss~\eqref{eq:true_metric} is minimized, then there will potentially be multiple primal variables $\tilde{\vec{z}}$, where $J_{0}(\vec{x}_{i},\tilde{\vec{z}}) = J_{0}^{*}(\vec{x}_{i})$. Graphically, these $\tilde{\vec{z}}$ is represented by the level set corresponding to $J_{0}^{*}(\vec{x}_{i})$, and naively minimizing~\eqref{eq:true_metric} will not be effective. As a result, we need to instead minimize a proxy loss function, where the minimizer of the proxy loss function is unique and corresponds to a minimizer of~\eqref{eq:true_metric} where each $\phi(\vec{x}_{i},\vec{\theta})|_{i=1}^{N_{B}}$ is primal feasible (assuming such a $\vec{\theta}$ exists). 

\textbf{Primal $\ell_{2}$ loss}: The most straightforward proxy loss would be the $\ell_{2}$ error in the primal variable space:

\begin{equation}
\label{eq:least_squares}
\sum_{i=1}^{N_{B}}||\phi(\vec{x}_{i};\vec{\theta}) - \vec{z}^{*}(\vec{x}_{i})||_{2}^{2}
\end{equation}

However, this proxy loss only indirectly minimizes the sub-optimality level through minimizing the distance between the predicted primal variables and the optimal primal variables. In addition, it is also only indirectly handling constraint satisfaction, since a penalty on violating the constraints does not appear in the loss function.


%is only a proxy to the metric we actually care, which is the sub-optimality level of our approximate open-loop parametric solution $J_{0}(\vec{x}(t),\) about is not how close $\vec{z}^{\phi}$ is to $\vec{z}^{*}$ in the $\ell_{2}$ distance in the primal variable space, but rather the difference in the open-loop predicted \textit{values} $J_{0}(\vec{x}, \vec{z}^{\phi})$ and $J_{0}(\vec{x},\vec{z}^{*})$. For example, to achieve asymptotic stability of our proposed control law, we need to achieve a certain sub-optimal error in terms of the open-loop value corresponding to the primal variables, not in terms an error in terms of the goodness-in-fit in the primal variable space. Thus we would like the minimize the $\ell_{2}$ error in the values corresponding to the predicted primal variables and the optimal primal variables:

%\begin{equation}
%\label{eq:least_squares_value}
%\argmin_{\vec{\theta}}\sum_{i=1}^{N_{B}}(J_{0}(\vec{x}_{i}, \vec{z}^{\phi}) - J_{0}(\vec{x}_{i},\vec{z}^{*}))^{2}
%\end{equation}

Instead, we used the Lagrangian proxy loss defined in Eqn.~\eqref{eq:least_squares_Lagrangian}. This loss is more appealing than the primal $\ell_{2}$ loss in~\eqref{eq:least_squares} since there is a direct connection between the Lagrangian and the value functions. Specifically, the optimal Lagrangian value corresponds to optimal value. As a result, using this proxy loss is directly minimizing the sub-optimality level, while still having the properties of uniqueness under constraint satisfaction. In addition, this proxy loss explicitly handles constraint violations. This explicit handling is not only theoretically appealing, but is also practically useful because we can directly manipulate the dual variables $(\lambda, \nu)$, while still maintaining dual feasibility, in order to obtain a more conservative neural network that is more likely to be primal feasible.

%The additional requirement when using this proxy loss is that when we generate our dataset, we need to additionally retain the dual variables. As a result, we need to generate tuples $\{\vec{x}, \vec{z}^{*}(\vec{x}), \vec{\lambda}^{*}(\vec{x}), \vec{\nu}^{*}(\vec{x})\}_{i=1}^{N_{B}}$. However, these additional dual variables are acquired for free when solving the implicit MPC problem with a primal-dual method, such as \textit{Mehrotra's Predictor-Corrector} method~\cite{mehrotra1992implementation}, and thus there is no additional work required to compute these variables when generating the dataset.



%\subsection{Dataset Generation}
%
%We use a supervised learning method to train the neural network $\vec{\phi}(\vec{x};\vec{\theta})$. This approach consists of generating a dataset $\{\vec{x}, \vec{z}^{*}(\vec{x})\}_{i=1}^{N_{B}}$ of states and the corresponding optimal primal variables. Since our labels $\vec{z}^{*}(\vec{x})$ are continuous variables, our supervised learning problem is a \textit{regression} problem. If the labels correspond to a finite set, the problem would be a \textit{classification} problem.
%
%Generating a dataset thus requires an \textit{oracle} to determine the label $\vec{z}^{*}(\vec{x})$ given an example $\vec{x}$. For example, for deep learning applications in computer vision, the oracle might be a human who provides labels for each example. As a result, the supervised learning framework can be \textit{expensive} since it is difficult for a human to label a large number of training instances.
%
%However for our problem of fitting the neural network to the optimal primal variables, our \textit{oracle} consists of a quadratic program solver to solve for $\vec{z}^{*}(\vec{x})$ for a given $\vec{x}$, which is relatively cheap since no human is needed to provide labels, and the quadratic program can be solve din finite time. It essentially becomes solving implicit MPC for multiple training examples. Thus the supervised framework is a good machine learning framework to apply for our problem.
%
%Solving implicit MPC fast is thus still of large importance in our framework so that we can generate a large dataset quickly. Usually in fast implicit MPC literature, the MPC solvers focus on \textit{latency}, or the ability to solve a single instance of the QP quickly. It is clear that due to our dataset approach, we care more about the \textit{throughput}, or our ability to solve a large number of problems quickly, of our solver, rather than it's latency. This is a subtle difference, but is also of importance because it allows us to utilize the inherent parallel structure of the dataset construction problem in a parallel computation framework to greatly speed up the data generation process over a naive implementation that simply solves for each training example sequentially.

%\subsection{Active Set Method}
%Duality theory and the usage of the Lagrangian allows us to handle constraints during training by minimizing the difference in the values corresponding to the predicted primal variables and the optimal primal variables. However, the neural network $\phi(\vec{x};\vec{\theta})$ is an approximation to the optimal control law $\vec{\mu}^{*}(\vec{x})$, and due to a variety of variables, such as the the non-convexity of the optimization problem~\eqref{eq:least_squares_Lagrangian} and the finite size of the dataset, there is no guarantee that the resulting learned neural network approximation will output feasible $\vec{z}^{\phi}$ for all feasible $\vec{x}$. In addition, while we can compute an upper bound on the sub-optimality of a specific $\vec{z}^{\phi}$ for a given $\vec{x}$ by computing the duality gap, we cannot compute a global upper bound. As a result, a secondary step is required to guarantee feasibility, a global sub-optimality bound, and thus asymptotic stability of the proposed control law.
%
%The secondary step that we use is the \textit{active set method}. Active set methods solve a sequence of equality-constrained quadratic subproblems. The goal of these methods is the predict the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*}, \vec{x})$ that are tight, or satisfied with equality, at the optimal solution. The reason why we utilize this method over an alternative method to solve for the quadratic program are that these methods are well suited to \textit{warm-starts}, where a good initial guess of $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*}, \vec{x})$ can speed up the optimization method. On the other hand, path-following methods such as interior point methods like Mehrotra's Predictor Correct, are not well suited for warm-starts, since the warm-start point can be far away from the path, and as a result, many iterates are needed to get the initial point back on the path. 
%
%Most active set methods require an initial feasible point. They thus consist of two phases, a \textit{Phase 1} method that finds an initial feasible point, and a \textit{Phase 2} method that takes this initial feasible point and performs the active set method algorithm. Given a $\tilde{\vec{z}}$ that is not too infeasible, the work required by the \textit{Phase 1} will be reduced~\textcolor{red}{cite Nocedal}. In addition, given a $\tilde{\vec{z}}$ that is close to $\vec{z}^{*}$, the work required by the \textit{Phase 2} method will also be reduced.


%Our approach utilizes the framework of the active set method to convert the approximate explicit MPC problem from a regression task to a classification task. Rather than learning to directly map the state parameters to control inputs, or a sequence of control inputs, we instead map the state parameters to the set of optimal active constraints. This is a supervised learning multi-label, multi-class classification problem.
%
%Once we have identified the optimal set of active constraints $\mat{G}_{\mathcal{A}}$, we can convert~\eqref{eq:decoupled_batch_problem} into a smaller equality-constrained sub-problem, of which we can solve closed-form by solving the following linear system of equations:
%
%\begin{equation}
%\label{eq:KKT_system}
%\left[
%\begin{array}{cc}
%2\bar{\mat{H}}^{T} & \mat{G}_{\mathcal{A}}^{T} \\
%\mat{G}_{\mathcal{A}} & 0\\
%\end{array} \right] \\
%\left[
%\begin{array}{c}
%\vec{z} \\
%\vec{\nu} \\
%\end{array} \right] = 
%\left[
%\begin{array}{c}
%0 \\
%\vec{f}_{\mathcal{A}} \\
%\end{array} \right]
%\end{equation}
%
%However, while we hope that the neural network will be able to correctly classify the optimal active set, it will most likely not completely correctly classify all of the active constraints. As a result, we utilize the output of the neural network to warm-start the active set method until some $\epsilon$-level of sub-optimality is achieved. The idea is that the neural network only misclassifies a few constraints, and as a result, only a few iterations of the active set method are needed until termination.
%
% uses a neural network to identify the constraints part of the optimal active set given the parameter $\vec{x}(t)$. This problem can be viewed as a \textit{multi-label}, \textit{multi-class} classification problem. It will thus be able to provide us with a good initial working set $\mathcal{W}$, which we can then use to warm-start an active-set method, which we will run until some predefined $\epsilon$ level of sub-optimality is achieved. This will allow us to provide guarantees on the persistent feasibility and sub-optimality of the neural network. 
%
%In addition, using the neural network to classify the active sets, which we then use to derive a control law, rather than directly representing some control law or value function, retains much of the problem structure. 
%
%Active set methods solve a sequence of equality-constrained quadratic subproblems. The goal of these methods is the predict the optimal active set $\mathcal{W}_{\mathcal{A}}$ that are tight, or satisfied with equality, at the optimal solution. An advantage of these methods are that they are well suited to \textit{warm-starts}, where a good initial guess of $\mathcal{W}_{\mathcal{A}}$ can speed up the optimization method. This is different than interior point methods, a path-following method, which are not well suited for warm-starts, as the warm-start point can be far away from the path, and as a result, many iterates are needed to get this initial point back on the path. As a result, for our paradigm of an offline trained neural network followed by a sequence of online optimization iterates, the active set method is a better framework.



==> tex/DoubleIntegratorResults.tex <==
\section{Double Integrator Results}

\subsection{Dataset Generation}
The double integrator dataset generation statistics are shown in Fig.~\ref{fig:training_stats}. The dataset generation time is the total time used to generate sobol sequence, train, test seed and test sets. 

\subsection{Training}
The neural network is comprised of three fully connected layers with units and activation functions shown in Table.~\ref{table:nn_structure}. The network is trained with Adam optimizer and Lagrangian loss for 100 epochs. We also monitor the l2 loss between the predicted and optimal primal variables, the predicted Lagrangian estimate and the optimal Lagrangian estimate during training. These quantities are also evaluated on a small held-out validation set.

%\begin{table}[h!]
%\centering
%    \begin{tabular}{|| c | c | c ||}
%        \hline\hline
%        Layer & Units & Activation  \\
%        \hline
%        1 & 32 & ReLU \\
%        \hline
%        2 & 32 & ReLU \\
%        \hline 
%        3 & 30 & None \\
%        \hline\hline 
%    \end{tabular}
%    \caption{Neural network structure for double integrator}
%    \label{table:nn_structure}
%\end{table}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/double_integrator/lagrangian_loss.png}
        \caption{Lagrangian loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/double_integrator/l2_loss.png}
        \caption{L2 loss}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/double_integrator/training_lagrangian_estimate.png}
        \caption{Lagrangian estimate in training}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/double_integrator/validation_lagrangian_estimate.png}
        \caption{Lagrangian estimate in validation}
    \end{subfigure}
    \caption{Double Integrator training stats}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillating_masses/lagrangian_loss.png}
        \caption{Lagrangian loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillating_masses/l2_loss.png}
        \caption{L2 loss}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillating_masses/training_lagrangian_estimate.png}
        \caption{Lagrangian estimate in training}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillating_masses/validation_lagrangian_estimate.png}
        \caption{Lagrangian estimate in validation}
    \end{subfigure}
    \caption{Oscillating masses training stats}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/quadrotor/lagrangian_loss.png}
        \caption{Lagrangian loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/quadrotor/l2_loss.png}
        \caption{L2 loss}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/quadrotor/training_lagrangian_estimate.png}
        \caption{Lagrangian estimate in training}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/quadrotor/validation_lagrangian_estimate.png}
        \caption{Lagrangian estimate in validation}
    \end{subfigure}
    \caption{Quadrotor training stats}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/high_dim_oscillating_masses/lagrangian_loss.png}
        \caption{Lagrangian loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/high_dim_oscillating_masses/l2_loss.png}
        \caption{L2 loss}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/high_dim_oscillating_masses/training_lagrangian_estimate.png}
        \caption{Lagrangian estimate in training}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/high_dim_oscillating_masses/validation_lagrangian_estimate.png}
        \caption{Lagrangian estimate in validation}
    \end{subfigure}
    \caption{High dimensional oscillating masses training stats}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/double_integrator/et_iterations_histogram.png}
        \caption{Double integrator}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillating_masses/et_iterations_histogram.png}
        \caption{Oscillating masses}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/quadrotor/et_iterations_histogram.png}
        \caption{Quadrotor}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/high_dim_oscillating_masses/et_iterations_histogram.png}
        \caption{High dimensional oscillating masses}
    \end{subfigure}
    \caption{Early termination acitve set iterations}
    \label{fig:et_iter_hist}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/double_integrator/optim_iterations_histogram.png}
        \caption{Double integrator}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/oscillating_masses/optim_iterations_histogram.png}
        \caption{Oscillating masses}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/quadrotor/optim_iterations_histogram.png}
        \caption{Quadrotor}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/high_dim_oscillating_masses/optim_iterations_histogram.png}
        \caption{High dimensional oscillating masses}
    \end{subfigure}
    \caption{Optimal termination acitve set iterations}
    \label{fig:optim_iter_hist}
\end{figure*}


\subsection{Testing}
We compare cold and warm starts methods with early termination or termination until result is optimal. Testing statistics are shown in Fig.~\ref{fig:test_stats}. Histograms of the number of active set iterations are shown in Fig.




==> tex/Feasibility.tex <==
\section{Ensuring Feasibility}

\begin{figure}[t!]
\centering
\includegraphics[width=.5\textwidth]{fig/Central_Path_Projection.png}
\caption{\textbf{Central Path Projection}}
\label{fig:central_path_projection}
\end{figure}

Our neural network approximation will not give us the exact solution, but rather a solution that is close to the exact solution in terms of the $\ell_{2}$ metric. If the optimal solution $\vec{U}_{0}^{*}$ lies on the boundary of the primal feasible region, then our neural network will likely output a solution $\tilde{\vec{U}}_{0}^{*}$ that is infeasible. Without an additional mechanism to project this potentially infeasible output back into this primal feasible region, our neural network will output a primal infeasible solution, and thus an infeasible control sequence for our optimal control problem~\eqref{eq:time_invariant_finite_horizon_problem}. Note that all of these projections will be occurring in the coupled batch problem.

The inequalities in Problem~\eqref{eq:coupled_batch_problem} $\mat{G}_{0}\vec{U}_{0} \leq \vec{w}_{0} + \mat{E}_{0}\vec{x}(t)$ are the $\mathcal{H}$-representation of the primal feasible polyhedra $\mathcal{F}_{0}$. One option is to compute the \textit{orthogonal projection} of $\tilde{\vec{U}}_{0}^{*}$ onto $\mathcal{F}_{0}$, which results in solving the following QP:

\small
\begin{equation}
\label{eq:orthogonal_projection}
\begin{aligned}
& \underset{\vec{U}_{0}}{\text{argmin}}  
& & J_{\textrm{OP}}(\vec{U}_{0}, \tilde{\vec{U}}_{0}^{*}) = \frac{1}{2}(\vec{U}_{0} - \tilde{\vec{U}}_{0}^{*})^{T}(\vec{U}_{0} - \tilde{\vec{U}}_{0}^{*}) \\
& \text{s.t.}
& & \mat{G}_{0}\vec{U}_{0} \leq \vec{w}_{0} + \mat{E}_{0}\vec{x}(t)\\
\end{aligned}
\end{equation}
\normalsize
which yields the primal feasible point $\hat{\vec{U}}_{0}^{\textrm{OP}}$ that is closest in the $\ell_{2}$ metric to the neural network output $\tilde{\vec{U}}_{0}$. Using this approach would involve solving a QP with the same computational complexity as solving~\eqref{eq:coupled_batch_problem}, which is not desirable. In addition, minimizing the $\ell_{2}$ norm is somewhat arbitrary.

As a result, we propose an alternative approach to project $\tilde{\vec{U}}_{0}^{*}$ onto $\mathcal{F}_{0}$. If $\tilde{\vec{U}}_{0}^{*} \in \mathcal{F}_{0}$, then it is obvious that no additional operation is necessary. Thus, we can assume that $\tilde{\vec{U}}_{0}^{*} \not\in \mathcal{F}_{0}$. The key idea is that if we can find another point $\vec{U}_{0, feas} \in \mathcal{F}_{0}$, then by searching along the line segment $L(\tilde{\vec{U}}_{0}^{*}, \vec{U}_{0, feas}) = \{ \tilde{\vec{U}}_{0}^{*} + \gamma \vec{U}_{0, feas} | ~\gamma \in [0,1]\}$, we can find a point $\vec{U}_{0} \in L(\tilde{\vec{U}}_{0}^{*}, \vec{U}_{0, feas})$ that is closest to $\ell_{2}$ norm to $\vec{U}_{0}$ while also being primal feasible. This point $\hat{\vec{U}}_{0}$ can be found in closed form by computing the intersection between a line segment and the boundary of the polyhedra, or even more simply by using a line search method to find an approximate solution. A solution is guaranteed to exist because one end of the line segment lies inside the polyhedra. \textcolor{red}{Write out the closed form solution, or the line search method. Make analogy to the backtracking line search, and how the line segment gives us a "search direction"}.

The difficulty is in finding the candidate $\vec{U}_{0, feas}$. One approach would be to solve a feasibility problem, which also has the same computational complexity as solving~\eqref{eq:coupled_batch_problem}, so is also not desirable. However, an alternative is rather than having our neural network only approximate the optimal solution $\vec{U}_{0}^{*}$, we can have it approximate a discrete set of central points $\vec{U}_{0}^{\kappa_{i}}$ for $i \in \{1, \dots,  n_{k}\}$, where $\vec{U}_{0}^{\kappa_{n_{k}}} = \vec{U}_{0}^{*}$.

For large $\kappa_{i}$, the central points $\vec{U}_{0}^{\kappa_{i}}$ approaches the \textit{analytic center} $\vec{U}_{0}^{ac}$ of $\mathcal{F}_{0}$. Intuitively, the analytic center is the point that is furthest away from the boundaries of $\mathcal{F}_{0}$. Recall that the reason that our neural network may output infeasible solutions is that $\vec{U}_{0}^{*}$ lies close to the boundary of $\mathcal{F}_{0}$, and thus $\tilde{\vec{U}}_{0}^{*}$ is likely lie outside of $\mathcal{F}_{0}$ due to approximation error. However for smaller $\kappa_{i}$, the central point $\vec{U}_{0}^{\kappa_{i}}$ will be more "central", or "embedded" in $\mathcal{F}_{0}$, and as a result, even with some approximation error, the network output $\tilde{\vec{U}}_{0}^{\kappa_{i}}$ will likely still be in $\mathcal{F}_{0}$. Thus we can find the largest $i$ such that $\tilde{\vec{U}}_{0}^{\kappa_{i}} \in \mathcal{F}_{0}$, and choose that to be $\mathbb{•}{U}_{0,feas}$. One drawback of this approach, are that there are no guarantees that for the learned neural network, there exists an $i$ such that $\tilde{\vec{U}}_{0}^{\kappa_{i}} \in \mathcal{F}_{0}$. However, in practice this occurrence is rare, and even it occurs, this method will be able to detect it and switch to an alternative approach.





==> tex/ObtainingGuarantees.tex <==
\section{Obtaining Guarantees with Online Primal Active Set Solver}
\label{sec:active_set}
%While the minimization of the Lagrangian loss function~\eqref{eq:lagrangian} during training will penalize constraint violations using optimal dual variables, the trained neural network will still potentially violate constraints since it is an approximation. This problem will be exacerbated as the dimensionality of the problem increases, and practically we see that for all problem the neural network will almost always output a primal infeasible approximation.

%The following intuitively describes why we will expect to see why an approximation will almost always output a primal infeasible solution. Intuitively, given an intial state parameter $\vec{x}$, unless the optimal primal variable $\vec{z}^{*}$ lies completely in the interior of the polyhedra defined by the inequality constraints of the QP, which is unlikely in meaningful cases because it means that the constraints have no effect on the QP, the solution will lie on the boundary of the polyhedra. The specific faces of the polyhedra that $\vec{z}^{*}$ lies on is defined by halfspace constraints or rows $\mat{G}_\textrm{0,eq}$ that are \textit{active}, which is a concept that will play a large role in our approach.
%
%
%Suppose that there are $n_{A}$ active constraints at $\vec{z}^{*}$. Let the event $A_{i} := \mat{G}^{i}_{0,\textrm{in}}\vec{z} \leq \vec{w}^{i}_{0,\textrm{in}} + \mat{E}^{i}_{0,\textrm{in}}\vec{x}$ for a given active constraint $i < n_{A}$. Since, $\vec{z}$ is an approximation, the probability $\mathbb{P}(A_{i}) < 1$. Since the rows of $\mat{G}_{0,\textrm{in}}$ are linearly independent, $\mathbb{P}(A_{j} | A_{i}) < 1$. As a result, $\mathbb{P}(A_{i}) \cap \mathbb{P}(A_{j})  = \mathbb{P}(A_{i})\mathbb{P}(A_{j} | A_{i}) < \mathbb{P}(A_{i})$ for $i \neq j$. For $\vec{z}$ to be primal feasible, we need $\cap_{i=1}^{n_{A}} A_{i}$, and we can see that $\mathbb{P}(\cap_{i=1}^{n_{A}} A_{i}) \rightarrow 0$ as $n_{A} \rightarrow \infty$, or when the problem dimensionality increases.  

%For a planner $\pi$ represented solely by an offline trained neural network $\phi$, it is a challenging to guarantee that both certificates of primal feasibility and suboptimality are satisfied for all states $\vec{x} \in \mathcal{X}_{0}$.  Most guarantees that can be provided on neural networks will be statistical~\cite{hertneck2018learning}, as there will be a chance that the neural network outputs an extremely poor prediction. 

We use an online method to ensure satisfaction of these conditions for all states $\vec{x} \in \mathcal{X}_{0}$. We utilize a primal active set solver~\cite[Ch. 16]{wright1999numerical} because it is distinguished among QP solver techniques in that it can be accelerated through warm starts from good initializations from the neural network, and it can also be terminated early once the certificates of primal feasibility and suboptimality are achieved. Methods such as interior-point methods are difficult to warm start~\cite{john2008implementation}, and other non-primal active set methods do not guarantee primal feasibility of intermediate iterates and cannot be terminated early~\cite{Ferreau2008}. Intuitively, the neural network removes the early iterations of the solver, and checking the criteria of Thm.~\ref{thm:approximate_RHC_stability} removes the final iterations.


%For these reasons, we employ a primal active set method as the online procedure. The primal active set method by itself can solve QP~\eqref{eq:decoupled_batch_problem}, which would be an \textit{implicit MPC} approach. We use the neural network output to warm-start the active set method, which intuitively cuts out steps from the beginning of the online procedure. We choose the primal version of the active set method in order to ensure intermediate primal variables are feasible, allowing us to terminate the algorithm as soon as the sub-optimality condition is met, which intuitively cuts out steps at the end of the online procedure. We are thus left with only performing the steps in the middle of the active set method that applies a few corrective steps to the neural network output. Our approach can thus be viewed as a hybrid \textit{explicit}-\textit{implicit} method. Before describing the process of integrating the neural network with the online procedure, we introduce the basic concepts behind the primal feasible active set solver.

\subsection{Warm Starting and Early Termination}
\label{sec:warm_starting_and_early_termination}
%There are a variety of optimization solvers for QPs, but there are two solver criteria that our proposed approach requires: (1) Ability to effectively use warm and hot-starts; and (2) Ability to terminate early and achieve a primal-feasible solution. The idea of warm and hot starts is to use the solution of a closely related QP to initialize the solver of the current QP to reduce computation time. Using no information from a previous solution to initialize the solver is called a cold start. The difference between a warm and hot start is specific to the particular solver algorithm and implementation, but the warm start typically only initializes part of the solver state such as the primal variables or basis factorization, while the hot start initializes all of the solver state.

%Many commercial solvers use interior-point methods \textcolor{red}{(cite Gurobi, CPlex)}, which follow a central path to an optimal solution \textcolor{red}{(cite Mehrotra textbook)}. However, these methods are not suitable for warm and hot starts, as the optimal solution from the previous problem will be far from the central path of the new problem and there will be many wasted iterations to get back onto the central path. In addition, the previous optimal solution may be near the constraint boundaries of the current problem, which can lead to numerical difficulties and degenerate, small steps \textcolor{red}{(cite)}. 



%These solvers are closely related to the concept of working sets introduced in Sec.~\ref{sec:guarantees_certificates}, as they explicitly maintain and update $\mathcal{W}_{\mathcal{A}}$, where each intermediate working set represents an equality-constrained quadratic subproblem. The goal of these procedures is to determine the optimal working set $\mathcal{W}^{*}_{\mathcal{A}}$, after which solving the corresponding KKT system~\eqref{eq:equality_constrained_KKT} will yield the optimal primal $\vec{z}^{*}$ and dual $\vec{\nu}^{*},\vec{\lambda}^{*}$ variables.

% Each row $i$ of the constraints in QP~\eqref{eq:decoupled_batch_problem} are active or inactive at a primal feasible solution. The goal of these methods is to determine the optimal working set $\mathcal{W}^{*}_{\mathcal{A}}$ consisting of those constraints that are tight, or satisfied with equality, at the optimal solution. 
%
%If $\mathcal{W}^{*}_{\mathcal{A}}$ is known in advance, then the solution for QP~\eqref{eq:decoupled_batch_problem} can found by solving the following equality-constrained QP:
%
%\begin{equation}
%\label{eq:equality_constrained_active_Set}
%\begin{aligned}
%& \underset{\vec{z}}{\text{argmin}}  
%& & J_{0}(\vec{z};\vec{x}(t)) =  \vec{z}^{T}\mat{H}\vec{z} + \vec{x}(t)^{T}\mat{Q}\vec{x}(t)\\
%& \text{s.t.}
%& & \vec{G}_{A}\vec{z} = \vec{w}_{A} +  \mat{E}_{A}\vec{x}(t),\\
%\end{aligned}
%\end{equation}
%
%The solution to this equality-constrained QP can be obtained by solving the KKT system
%
%The left matrix in Eqn.~\eqref{eq:equality_constrained_KKT} is called the \textit{KKT} matrix. Positive definiteness of $\mat{H}$ and full row rank of $\mat{G}_{A}$, conditions which are satisfied in our case, imply that the KKT matrix is invertible, and thus the equality constrained QP~\eqref{eq:equality_constrained_active_Set} has a closed-form solution.
% 
%The problem is that $\mathcal{W}^{*}_{\mathcal{A}}$ is usually not known in advance, and the purpose of active set methods is determination of this set. It is clear that all equality constraints must be in $\mathcal{W}^{*}_{\mathcal{A}}$, otherwise the optimal active set corresponds to a region that does not contain primal feasible variables. Thus the active set method explicitly identifies which of the inequality constraints will be active at the optimal solution. 


Active set methods solve inequality-constrained QPs by solving a sequence of equality-constrained quadratic subproblems~\cite{wright1999numerical}. The general approach is to start with some initial guess of the active constraints, and proceed by adding and removing constraints until the optimal solution is found. Active set methods are well-suited to acceleration due to good initalization~\cite{wright1999numerical}. 

As a result, our algorithm speeds up online computation in two ways. First, by using the neural network primal prediction $\vec{z}$, we can warm-start the solver. Second, by checking for the feasibility and stability certificates using the efficient methods provided in Sec.~\ref{sec:certificates_feasibility_suboptimality}, we can terminate the online solver early. In order to take advantage of both of these methods, we use a primal active set solver. These solvers explicitly find and maintain primal feasibility of intermediate iterates, which is necessary to satisfy the certificate of primal feasibility prior to reaching optimality. They are split into two phases. In \textit{Phase I}, the solver first finds an initial primal feasible point by solving a linear feasibility program, which provides the certificate of primal feasibility. Starting from this primal feasible point, \textit{Phase II} updates the primal solution and the active constraints while maintaining primal feasibility.  During this phase, we check the duality gap at the intermediate iterates using the techniques described in Sec.~\ref{sec:guarantees_certificates} in order to obtain the certificate of suboptimality.

\begin{algorithm}[t]
	\caption{Explicit-Implicit Planner}
	\label{alg:explicit_implicit_planner}
	\begin{algorithmic}[1]
	\Procedure{$ExplicitImplicitPlanner$}{$\tilde{\vec{\theta}}, \vec{x}, \mathcal{A}$}
		\State $\backslash \backslash~\vec{x}$ is the initial state parameter
		\State $\backslash \backslash~\tilde{\vec{theta}}$ are the neural network parameters 
		\State $\backslash \backslash~\mathcal{A}$ is the primal active set solver
		\State $\backslash \backslash$ \textbf{Explicit}
		\State Obtain neural network prediction $\tilde{\vec{z}}$
		\State $\backslash \backslash$ \textbf{Implicit}
		\State Obtain certificate of primal feasibility and \\ \hspace{4mm} suboptimality according to Sec.~\ref{sec:certificates_feasibility_suboptimality}.
		\If {both certificates obtained}
			\State \Return $\tilde{\vec{z}}$
		\Else
			\State Warm start $\mathcal{A}$ with $\tilde{\vec{z}}$ according to Sec.~\ref{sec:warm_starting_and_early_termination}. 
			\State Perform \textit{Phase I} of $\mathcal{A}$ and obtain certificate of \\ \hspace{6mm} primal feasibility
			\While {no certificate of suboptimality}
				\State Update $\tilde{\vec{z}}$ via \textit{Phase II} iteration of $\mathcal{A}$.
				\State Check certificate of suboptimality \\ \hspace{8mm} according to Sec.~\ref{sec:certificates_feasibility_suboptimality}.
			\EndWhile
	
		\State \Return $\tilde{\vec{z}}$
		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

Our final hybrid explicit-implicit algorithm that computes approximate planner $\hat{\pi}$ is described in Alg.~\ref{alg:explicit_implicit_planner}. This procedure is guaranteed to terminate in finite time as the active set method will reach the optimal solution in finite time~\cite[Ch. 16]{wright1999numerical}. In addition, for all $\vec{x} \in \mathcal{X}_{0}$, $\hat{\pi}$ will obtain a certificate of primal feasibility and suboptimality. As a result, given that the terminal constraint and terminal cost were chosen to satisfy the conditions specified in Thm.~\ref{thm:approximate_RHC_stability}, the resulting $\hat{\mu}$ is guaranteed to be recursively feasible and asymptotically stable according to Thm.~\ref{thm:approximate_RHC_stability}.



%\subsection{Estimating the Working Set}
%
%In order to use the active set method to correct the neural network, we will use the network output $\tilde{\vec{z}}$ to warm start the active set solver by initializing part of the solver state. In addition to the primal variables, active set methods typically need an estimate of the working set $\tilde{\mathcal{W}}_{\mathcal{A}}(\vec{x})$ for a warm start.
% 
%While one option is to additionally predict which constraints are in $\tilde{\mathcal{W}}_{\mathcal{A}}(\vec{x})$, this will substantially increase the size of the neural network, and is not desirable. In addition, separately predicting these variables is redundant, as we can use the QP problem structure to derive an estimate of the working set from the primal variables. 
%
%
%
%Alg.~\ref{alg:estimate_basis_variables} demonstrates one approach to estimate the working set $\tilde{\mathcal{W}}_{\mathcal{A}}$ from the primal variables $\tilde{\vec{z}}$. The constraints that correspond to equality constraints must be active at the optimal solution, and are thus included into $\tilde{\mathcal{W}}_\mathcal{A}(\vec{x})$. The active status of the inequality constraints can be evaluated by plugging in the predicted primal variables into inequality constraint matrix. If the primal variables lie near a constraint by a certain margin specified by $\delta$, then it is deemed to be active and included into $\tilde{\mathcal{W}}_\mathcal{A}(\vec{x})$. The choice of $\delta$ is a parameter that can be tuned. For the optimal primal variables $\vec{z}^{*}$, any $\delta \geq 0$ will yield the optimal working set $\mathcal{W}^{*}_{\mathcal{A}}(\vec{x})$.
%
%Given an initial state $\vec{x}$, the neural network estimates $\tilde{\vec{z}}$. Using Alg.~\ref{alg:estimate_basis_variables}, we can use $\tilde{\vec{z}}$ to estimate the working set $\tilde{\mathcal{W}}_{\mathcal{A}}$. Together, $\tilde{\vec{z}}$ and $\tilde{\mathcal{W}}_{\mathcal{A}}$ can be used to warm start the active set method.
%
%\subsection{Early Termination with Guarantees}
%
%
%
%By using a primal feasible active set method, upon early termination, as long as we are in \textit{Phase II} of the active set algorithm, we can ensure that our primal variables will be primal feasible, and thus obtain the guarantee on recursive feasibility. This ability to guarantee primal feasibility during early termination is the key reason why it is necessary to use a primal feasible active set method, rather than a parametric active set method, which only guarantees primal feasibility at the optimal solution.




%In order to guarantee asymptotic stability, we compute the feasible duality gap which is an upper bound of the sub-optimality level. The feasible duality gap is easy to compute once we have feasible primal variables and feasible dual variables. Our primal feasible active set method already provides feasible primal variables. However, the estimate of the dual variables may be infeasible, and the dual cost computed from infeasible dual variables is not necessarily a lower bound to the optimal cost. The role of the dual variable is to simply provide a certificate for asymptotic stability, and they are not used in the actual closed-loop implementation of the RHC. As a result, when we encounter an infeasible dual iterate, we can project the dual variables onto the feasible dual region to obtain a valid lower bound on the optimal cost. 
%
%\begin{algorithm}[t]
%	\caption{Estimate Dual Variables}
%	\label{alg:estimate_dual_variables}
%	\begin{algorithmic}[1]
%	\Procedure{DUAL}{$\vec{x}$, $\vec{z}$, $\delta$}
%		\State $\backslash \backslash~\vec{x}$ is the initial state parameter
%		\State $\backslash \backslash~\vec{z}$ are the estimated primal variables
%		\State $\backslash \backslash \delta \in \mathbb{R}$ is a threshold parameter
%		\State $\vec{\beta} = [ \vec{\beta}_{\textrm{eq}}; \vec{\beta}_{\textrm{in}} ]  $ = BASIS($\vec{x}$, $\vec{z}$, $\delta$)
%		\State Set $[ \nu_{nb}; \lambda_{nb} ]$ as the elements of $[ \nu; \lambda ]$ that have corresponding $\beta$ that are non-basic.
%		\State Set $G_{nb}$ as the rows of $[G_{\textrm{eq}}; G_{\textrm{in}}]$ that have corresponding $\beta$ that are non-basic.
%		\State $\vec{\beta}_{\textrm{in}} = \mathds{1}(\vec{G}_{\textrm{in}}\vec{z} - \vec{w}_{\textrm{in}} + \mat{E}_{\textrm{in}}\vec{x} \geq -\delta \vec{1})$
%		\State $\vec{\beta} = [ \vec{\beta}_{\textrm{eq}}; \vec{\beta}_{\textrm{in}} ]$
%		\State \Return $\vec{\beta}$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}
%
%The feasible region for the inequality dual variables is defined by the non-negative orthant $\lambda \succcurlyeq \vec{0}$, while the feasible region for the equality dual variables $\nu$ is unconstrained. This specific shape of the dual feasible region allows us to easily peform the projection operation, as it is easy to perform an orthogonal projection operation onto the non-negative orthant by setting any negative inequality dual variable to $0$. On the other hand, it would not be as easy to project the primal variables onto its feasible region, as the orthogonal projection would be onto a polyhedra, which would involve solving another QP. 
%
%Once we obtain this feasible dual variable, we can then compute the duality gap, and terminate the algorithm once it gets below the first stage cost.
%
%\textcolor{red}{(Provide Overall algorithm of entire procedure?)}
%
%\begin{algorithm}[t]
%	\caption{Proposed Control Law}
%	\label{alg:proposed_control_law}
%	\begin{algorithmic}[1]
%		\Procedure{Sub-Optimal Control Law}{$\tilde{\pi}$, $\vec{x}$, $\mat{M}$}
%		\State $\backslash \backslash~ \phi(\vec{x};\vec{\theta})$ is the neural network
%		\State $\backslash \backslash~ \vec{x}$ is the current state
%		\State $\backslash \backslash~ \mat{M}$ is matrix defining contribution to the stage cost dependent on the state
%		\State $\gamma(\vec{x}) = \vec{x}^{T}\mat{M}\vec{x}$
%		\State $\vec{z}^{init} = \phi(\vec{x};\vec{\theta})$ \Comment{Call Neural Network}
%		\State Obtain $\vec{z}^{A}$ by calling Alg.~\ref{alg:active_set} with $\vec{z}_{init}$ and $\gamma(\vec{x})$
%		\State Implement the first control action $u_{0}^{A}$ in $\vec{z}^{A}$
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}





==> tex/OldResults.tex <==
\section{Results}
\begin{figure*}[t!]
\begin{center} 
 \setlength\extrarowheight{5pt}
 \resizebox{\textwidth}{!}
 {\begin{tabular}{||c | c| c| c ||} 
 \hline
 Measure & Feasible Control Law (Analytic Center) & Predicted Control Law (No Projection) & Final Control Law\\ [0.6ex] 
 \hline\hline
 Average Value Error & 91.4 (27.1 $\%$) & 0.16 (0.44 $\%$) & 2.58 (0.55 $\%$) \\
 \hline\hline
 Median Value Error & 91.8 (26.6 $\%$) & 0.10 (0.03 $\%$) & 0.12 (0.03 $\%$) \\
  \hline\hline
  Maximum Value Error & 83.9 $\%$ & 1.8 $\%$ & 31.5 $\%$ \\
  \hline\hline
 Number Find Feasible (29,970) & 25,122 (83.8 $\%$) & 24,881 (83.0 $\%$) & 27,456 (91.6 $\%$) \\
    \hline\hline
 Number $< 3\%$ error  & 0.0 $\%$  & 100 $\%$ & 94.4 $\%$ \\
    \hline\hline
\end{tabular}}
\end{center}
\caption{Results }
\label{fig:oscillating_masses}
\end{figure*}


\begin{figure*}[t!]
\begin{center} 
 \setlength\extrarowheight{5pt}
 \resizebox{\textwidth}{!}
 {\begin{tabular}{||c | c | c |c |c |c ||} 
 \hline
 Margin & Lagrangian Train {\tiny ($\# 451,266$)} & $\ell_{2}$ Train {\tiny ($\# 451,266$)} & Lagrangian Test {\tiny ($\# 29,868$)} & $\ell_{2}$ Test {\tiny ($\# 29,868$)} & No Dropout Test {\tiny ($\# 29,868$)} \\ [0.6ex] 
 \hline\hline
 0.00 & $0.0 \%$ {\tiny ($1$)}  & $0.0 \%$ {\tiny ($7$)}  & $0.0 \%$ {\tiny ($0$)}& $0.0 \%$ {\tiny ($0$)} & $0.0 \%$ {\tiny ($1$)}\\
 \hline\hline
 0.01 & $83.1 \%$ {\tiny ($375,120$)} & $82.1 \%$ {\tiny ($370,433$)}  & $83.5 \%$ {\tiny ($24,932$)} & $82.4 \%$ {\tiny ($24,621$)} & $85.0 \%$ {\tiny ($25,400$)} \\
  \hline\hline
  0.05 &  $88.1 \%$ {\tiny ($397,932$)} & $86.3 \%$ {\tiny ($389,625$)}  & $88.2 \%$ {\tiny ($26,367$)} & $86.6 \%$ {\tiny ($25,876$)} & $91.6 \%$ {\tiny ($27,362$)}\\
  \hline\hline
 0.10 &  $93.7 \%$ {\tiny ($422,904$)} & $90.9 \%$ {\tiny ($410,225$)} & $93.4 \%$ {\tiny ($27,905$)} & $90.9 \%$ {\tiny ($27,162$)} & $96.1 \%$ {\tiny ($28,715$)}\\
    \hline\hline
 0.15  &  $96.5 \%$ {\tiny ($435,523$)} & $94.3 \%$ {\tiny ($425,361$)} & $96.2 \%$ {\tiny ($28,745$)}  & $94.1 \%$ {\tiny ($28,131$)} & $98.1 \%$ {\tiny ($29,320$)}\\
    \hline\hline
 0.20  &  $98.1 \%$ {\tiny ($442,772$)}  &  $96.4 \%$ {\tiny ($435,201$)}  & $97.9 \%$ {\tiny ($29,235$)} & $96.4 \%$ {\tiny ($28,786$)} & $99.2 \%$ {\tiny ($29,636$)}\\
    \hline\hline
 0.25 &  $99.1 \%$ {\tiny ($447,347$)} & $97.9 \%$ {\tiny ($441,682$)} & $98.9 \%$ {\tiny ($29,536$)}  & $97.8 \%$ {\tiny ($29,225$)} & $99.7 \%$ {\tiny ($29,783$)} \\
    \hline\hline
 0.50  &  $100.0 \%$ {\tiny ($451,256$)}  &  $99.9 \%$ {\tiny ($450,909$)}     & $100.0 \%$ {\tiny ($29,867$)}& $99.9 \%$ {\tiny ($29,845$)} & $100.0\%$ {\tiny ($29,868$)}\\
    \hline\hline
 1.00  &  $100.0 \%$ {\tiny ($451,266$)} &  $100.0 \%$ {\tiny ($451,266$)}  & $100.0 \%$ {\tiny ($29,868$)} & $100.0 \%$ {\tiny ($29,868$)} & $100.0 \%$ {\tiny ($29,868$)}\\
    \hline\hline
\end{tabular}}
\end{center}
\caption{Percentage Feasible }
\label{fig:oscillating_masses}
\end{figure*}

\begin{figure*}[t!]
\begin{center} 
 \setlength\extrarowheight{5pt}
 \resizebox{\textwidth}{!}
 {\begin{tabular}{||c | c| c| c | c |c | c||} 
 \hline
 Measure & Lagrangian Train  & $\ell_{2}$ Train  & Lagrangian Test& $\ell_{2}$ Test & No dropout Test & Projected\\ [0.6ex] 
 \hline
 Average $\ell_{2}$ error (\textit{primal}) & 0.12 & 0.186 & 0.128  & 0.186 & 0.065 & 0.036\\
 \hline
 Median $\ell_{2}$ error (\textit{primal}) & 0.07 & 0.106 & 0.069  & 0.107 & 0.024 & 0.020 \\
  \hline
  Maximum $\ell_{2}$ error (\textit{primal}) & 8.52 & 11.84 & 4.35 & 6.16 & 4.42 & 1.45\\
  \hline\hline
   Average Value Error (\textit{cond. $< 0.01$ margin}) & 0.70 (0.18$\%$) & 1.58 (0.42$\%$) & 0.72 (0.19$\%$) & 1.58 (0.42$\%$) & 1.76 (0.46$\%$) & 1.16 (0.27$\%$)\\
   \hline
   Median Value Error (\textit{cond. $< 0.01$ margin}) & 0.48 (0.14 $\%$) & 1.32 (0.38 $\%$) & 0.48 (0.14 $\%$) & 1.33 (0.39 $\%$) & 1.36 (0.40 $\%$) & 0.70 (0.19 $\%$)\\
   \hline
   Max Value Error (\textit{cond. $< 0.01$ margin}) & 22.1 (5.1 $\%$) & 32.48 (4.3 $\%$) & 25.6 (5.7 $\%$) & 13.8 (2.6 $\%$) & 23.4 (5.6 $\%$) & 36.4 (5.4 $\%$)\\
   \hline
   Min Value Error (\textit{cond. $< 0.01$ margin}) & -29.4 (-6.6 $\%$) & -26.9 (-6.2$\%$) & -12.0 (-2.6$\%$) & -9.4 (-2.1$\%$) & -10.0 (-2,2$\%$) & 0.02 (0.0$\%$) \\
   \hline\hline
   Average Lagrangian Error (\textit{all}) & 0.58 (0.16 $\%$) & 0.64 (0.17 $\%$) & 0.61 (0.16 $\%$) & 0.65 (0.16 $\%$) & 0.22 (0.05 $\%$) & 0.11 (0.0 $\%$)\\
   \hline
   Median Lagrangian Error (\textit{all}) & 0.37 (0.12 $\%$) & 0.33 (0.11 $\%$) & 0.37 (0.12 $\%$) & 0.33 (0.11 $\%$) & 0.07 (0.02 $\%$) & 0.05 (0.01 $\%$)\\
   \hline
   Max Lagrangian Error (\textit{all}) & 51.3 ( 10.4 $\%$) & 77.0 (15.6 $\%$) & 25.7 (5.9 $\%$) & 41.4 (6.7 $\%$) & 21.06 (5.3 $\%$) & 7.32 (1.9 $\%$)\\
   \hline
   Min Lagrangian Error (\textit{all}) & 0.05 (0.0 $\%$) & 0.05 (0.0 $\%$) & 0.05 (0.0 $\%$) & 0.06 (0.0 $\%$) & 0.01 (0.0 $\%$) & 0.01 (0.0 $\%$)\\
  \hline\hline
\end{tabular}}
\end{center}
\caption{Results statistics }
\label{fig:oscillating_masses}
\end{figure*}

==> tex/ProblemFormulation.tex <==
\section{Problem Statement}
\label{sec:problem_statement}

Consider a discrete-time linear time-invariant system,
%
\begin{equation}
\label{eq:system}
\vec{x}(t+1) = \mat{A}\vec{x}(t) + \mat{B}\vec{u}(t),
\end{equation}
subject to a set of constraints,
\begin{equation}
\begin{aligned}
\label{eq:constraints}
\vec{x}(t) \in \mathcal{X} &:= \{\vec{x}\in \mathbb{R}^{n}|\mat{A}_{x}\vec{x} \leq \vec{b}_{x} \} \quad &\forall~t& \geq 0,\\
\vec{u}(t) \in \mathcal{U} &:= \{\vec{u}\in \mathbb{R}^{m}|\mat{A}_{u}\vec{u} \leq \vec{b}_{u} \} \quad &\forall~t& \geq 0.
\end{aligned}
\end{equation}
Assuming that the pair $(\mat{A},\mat{B})$ is stabilizable~\cite[Ch. 7]{borrelli2017predictive}, we are interested in obtaining a receding horizon controller (RHC)~\cite[Ch. 12]{borrelli2017predictive}. At each time step, we repeatly solve a constrained finite time optimal control problem~\cite[Ch. 7]{borrelli2017predictive} given by,
\begin{align}
& \min_{\vec{u}_{0:N-1}}  
& & J(\vec{u}_{0:N-1} | \vec{x}(t)) \stackunder[5pt]{{}= \vec{x}_{N}^{\top}\mat{P}\vec{x}_{N} {}}{ {}+ \sum_{k=0}^{N-1} \prl{\vec{x}_{k}^\top\mat{Q}\vec{x}_{k} +\vec{u}_{k}^\top\mat{R}\vec{u}_{k}}}\notag\\
& \quad\text{s.t.}
& & \vec{x}_{k+1} = \mat{A}\vec{x}_k +\mat{B}\vec{u}_k, \;\vec{x}_{0} = \vec{x}(t),\notag\\
& & & \mat{A}_{x}\vec{x}_k \leq \vec{b}_{x}, \mat{A}_{u}\vec{u}_k \leq \vec{b}_{u}, \mat{A}_{f}\vec{x}_{N} \leq \vec{b}_{f}\label{eq:time_invariant_finite_horizon_problem}
\end{align}
where $N$ is the horizon, and symmetric matrices $\mat{Q}, \mat{P} \in \mathcal{S}^n_{\succ 0}$, $\mat{R}\in\mathcal{S}^m_{\succ 0}$ are chosen to define the desired optimal behavior for the system. The terminal cost, $\vec{x}_{N}^{\top}\mat{P}\vec{x}_{N}$, and the terminal constraint set, $\mathcal{X}_{f} := \{\vec{x} \in \mathbb{R}^{n} | \mat{A}_{f}\vec{x} \leq \vec{b}_{f}\}$, ensure feasibility and asymptotic stability of the receding horizon controller as will be discussed in Sec.~\ref{sec:rhc}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Assume that the pair $(\mat{A},\mat{B})$ is stabilizable~\cite[Ch. 7]{borrelli2017predictive}. For a given state $\vec{x}(0)$, our goal is to compute a sequence of control inputs $\vec{u}_{0:\infty} := \{\vec{u}_{0}, \vec{u}_{1}, \dots\}$ to regulate the system to a desired state in the interior of the feasible set~\eqref{eq:constraints}. Without loss of generality, this desired state will be assumed to be the origin. This problem, known as the constrained infinite-horizon linear quadratic regulator (LQR) problem~\cite[Ch. 11]{borrelli2017predictive}, is:
%
%\begin{equation}
%\label{eq:general_problem}
%\begin{aligned}
%& \min_{\vec{u}_{0:\infty}}
%& & J(\vec{u}_{0:\infty},\vec{x}(0)) =  \sum_{k=0}^{\infty} \left(\vec{x}_k^{\top}\mat{Q}\vec{x}_k +\vec{u}_k^{\top}\mat{R}\vec{u}_k\right)\\
%& \;\;\text{s.t.}
%& & \vec{x}_{k+1} = \mat{A}\vec{x}_k +\mat{B}\vec{u}_k, \;\vec{x}_{0} = \vec{x}(0),\\
%& & & \mat{A}_{x}\vec{x}_k \leq \vec{b}_{x},\\
%& & & \mat{A}_{u}\vec{u}_k \leq \vec{b}_{u},
%\end{aligned}
%\end{equation}
%
%where the symmetric matrices $\mat{Q} \in \mathcal{S}^n_{\succ 0}$ and $\mat{R}\in\mathcal{S}^m_{\succ 0}$ are chosen to define the desired optimal behavior for the system. Note that $\vec{x}_{k}$ is a prediction of the state at time step $k$ and is an \textit{optimization} variable, while $\vec{x}(0)$ is the actual state at the current time $t=0$ and is a \textit{parameter}. When optimal behavior is needed at multiple initial states, instead of recomputing the input sequence $\vec{u}_{0:\infty}$ every time, it is desirable to obtain a control policy $\vec{\mu}^*(\vec{x})$ that specifies the optimal input for an arbitrary state $\vec{x}$.




%Consider a discrete-time linear time-invariant system 
%\begin{equation}
%\label{eq:system}
%\begin{aligned}
%&\vec{x}(t+1) = \mat{A}\vec{x}(t) + \mat{B}\vec{u}(t), \\
%&\vec{x}(t) \in \mathbb{R}^{n}\!, \; \vec{u}(t) \in \mathbb{R}^{m} \quad \forall~t \geq 0.
%\end{aligned}
%\end{equation}
%Our goal is to compute a sequence of control inputs $\{ \vec{u}_{0}, \vec{u}_{1}, \dots\}$ to regulate the system to a desired state subject to a set of constraints
%\begin{equation}
%\label{eq:constraints}
%\vec{x}(t) \in \mathcal{X}\!, \;  \vec{u}(t) \in \mathcal{U}, \quad \forall~t\geq 0
%\end{equation} 
%where $n$ is the state dimension, $m$ is the control inputs dimension, and $\mathcal{X}=\{\vec{x}|\mat{A}_{x}\vec{x} \leq \vec{b}_{x} \}$, $\mathcal{U} = \{\vec{u}|\mat{A}_{u}\vec{u} \leq \vec{b}_{u} \}$ are closed convex polyhedra which contain the origin in their interior. It is assumed that the pair $(\mat{A},\mat{B})$ is stabilizable. This problem, known as the constrained infinite-horizon LQR, is:
%\begin{equation}
%\label{eq:general_problem}
%\begin{aligned}
%& \underset{\vec{U}_{0 \rightarrow \infty}}{\text{argmin}}
%& & J_{\infty}(\vec{x}(0)) =  \sum_{k=0}^{\infty} \left(\vec{x}_k^T\mat{Q}\vec{x}_k +\vec{u}_k^T\mat{R}\vec{u}_k\right)\\
%& \text{s.t.}
%& & \vec{x}_{0} = \vec{x}(0) \\
%& & & \vec{x}_{k+1} = \mat{A}\vec{x}_k +\mat{B}\vec{u}_k, \\
%& & & \mat{A}_{x}\vec{x}_k \leq \vec{b}_{x} \\
%& & & \mat{A}_{u}\vec{u}_k \leq \vec{b}_{u}
%\end{aligned}
%\end{equation}
%where $\vec{U}_{0:\infty} = \{\vec{u}_{0}, \vec{u}_{1}, \dots\}$, $\mat{Q} \in \mathcal{S}^n_{\succeq 0}$ and $\mat{R}\in\mathcal{S}^m_{\succ 0}$ are chosen to define the desired optimal behavior for the system. Rather than computing the sequence of control inputs $\vec{U}_{0:\infty}$ for a given state $\vec{x}(0)$, our goal is to compute a control function $\vec{\mu}^*(\vec{x}(t))$ that specifies the optimal control input for an arbitrary state $\vec{x}(t)$ at time $t$. 


==> tex/ProposedControlLaw.tex <==
\section{Proposed Control Law}

We propose a procedure that computes an open loop mapping $\pi$ for the open-loop optimization problem~\eqref{eq:decoupled_batch_problem}, where the corresponding RHC $\pi_{0}$ is guaranteed to be recursively feasible and asymptotically stable. The procedure can be broken down into two components. A neural network $\phi(\vec{x};\vec{\theta})$ is first trained offline to approximate the optimal open loop mapping $\pi^{*}$ by minimizing the sub-optimality level $\sigma(\phi(\vec{x};\vec{\theta}); \vec{x})$ via a proxy loss based on the Lagrangian from duality theory. 

During online implementation of the control law, the neural network is called to obtain $\vec{z}_{init} = \phi(\vec{x};\vec{\theta})$, and an active set method is applied to $\vec{z}_{init}$ to obtain $\vec{z}_{A}$ where $\vec{z}_{A}$ is guaranteed to be primal feasible and $\sigma(\vec{z}_{A};\vec{x})$ is bounded by a prespecified $\gamma(\vec{x})~\forall \vec{x}$.. The combination of these two components defines the open loop mapping $\pi^{A}$, which is feasible and $\gamma$-optimal. As a result, the corresponding RHS $\pi_{0}^{A}$ is guaranteed to be recursively feasible and asymptotically  stable.

\subsection{Neural Network Architecture}

\begin{defn} (Deep Neural Network)
A deep neural network (\textit{DNN}) $\phi(\vec{x};\vec{\theta})$ with $L$ layers is a composition of $L$ affine functions
\begin{equation}
\label{eq:affine_layer}
\vec{\lambda}^{\phi}_j(\vec{x}) := \mat{\theta}^{W}_j\vec{x}+\vec{\theta}^{b}_{j},
\end{equation}
each except the last one followed by a nonlinear activation function $\vec{h}^{\phi}$, so that:
\[
\phi(\vec{x};\vec{\theta}) = \vec{\lambda}^{\phi}_{L} \circ \vec{h}^{\phi} \circ \vec{\lambda}^{\phi}_{L-1} \circ \cdots \circ \vec{h}^{\phi} \circ \vec{\lambda}^{\phi}_{1}(\vec{x}),
\]
where $\vec{\theta}:=\{\mat{\theta}^{W}_{1:L}, \vec{\theta}^{b}_{1:L}\}$ are the affine function parameters to be optimized, and $\vec{h}^{\phi}$ is a fixed (not optimized) function, typically chosen as a sigmoid, hypertangent, or rectified linear unit (ReLU) function (see~\cite[Ch.6]{Goodfellow-et-al-2016} for details).
\end{defn}

Previous work has made the connection between the constrained LQR problem and neural network with ReLu activation functions (DNN ReLu), $\vec{h}^{\phi}(\vec{x}) := \max\{0,\vec{x}\}$~\cite{Chen2018ApproximatingEM}. The optimal control law of the constrained LQR problem is a continuous PWA function on polyhedra, and the neural network with ReLu activation functions also compute continuous PWA function on polyhedra. 

In addition to DNN ReLu being universal approximators, there are a few theorems on characterizing the \textit{exact} representation of PWA on polyhedra functions by DNN ReLU that can be used as guidelines to design an appropriate network architecture for a specific problem. For example, every $\mathbb{R}^{n} \rightarrow \mathbb{R}$ continuous PWA on polyhedra function can be represented by a DNN ReLU with at most 
\begin{equation}
\label{eq:network_depth}
L = \ceil{\log_{2}(n+1)}+1
\end{equation} depth (layers)~\cite[Thm 2.1]{arora2016understanding}. 

This formula can be generalized to continuous PWA on polyhedra functions of arbitrary output dimension.

\begin{thm} (Exact Representation for Multivariate Range)
	Suppose $f:\mathbb{R}^{n} \rightarrow \mathbb{R}^{m}$ for $n,m \in \mathbb{N}^{+}$ is a continuous PWA on polyhedra function. Then $f$ can be exactly represented by a DNN ReLu with at most
	\begin{equation}
	\label{eq:generalized_etwork_depth}
		L = \ceil{\log_{2}(n+1)}+1
	\end{equation} depth
\end{thm}
\begin{pf}
	Let $f:\mathbb{R}^{n} \rightarrow \mathbb{R}^{m}$ be a continuous PWA on polyhedra function. We need to construct a DNN ReLu $\phi$ with at most $L = \ceil{\log_{2}(n+1)}+1$ layers that exactly represents $f$. Let $f_{i}:\mathbb{R}^{n} \rightarrow \mathbb{R}$ for $i=1,\dots,m$ represent the $i-th$ dimension of $f$, that is $f = f_{1} \times f_{2} \dots \times f_{m}$, where $\times$ denotes the Cartesian product. In other words when viewed as matrices, $f = [f_{1};\dots;f_{m}]$. By~\cite[Thm 2.1]{arora2016understanding}, each $f_{i}$ can be represented by a DNN ReLu $\phi_{i}$ with depth $L=\ceil{\log_{2}(n+1)}+1$. Let $\vec{\theta}_{j,i} = \{\vec{\theta}_{j,i}^{W},\vec{\theta}_{j,i}^{b}\}$ represent the parameters of $\vec{\lambda}_{j,i}^{\phi}$, the $j$-th layer of network $\phi_{i}$. 
	
	We will start with the first hidden layer of $\phi$, denoted $\vec{\lambda}_{1}^{\phi}$. Let $\vec{\theta}_{1}^{W} = [\vec{\theta}_{1,1}^{W}; \dots;\vec{\theta}_{1,m}^{W}]$, and likewise for  $\vec{\theta}_{1}^{b}$. These $\vec{\theta}_{1} = \{\vec{\theta}_{1}^{W}, \vec{\theta}_{1}^{b}\}$ define $\vec{\lambda}_{1}^{\phi}$ according to the affine function~\eqref{eq:affine_layer}. In addition, $\vec{\lambda}_{1}^{\phi} = [\vec{\lambda}_{1,1}^{\phi}; \dots;\vec{\lambda}_{1,m}^{\phi}]$.
	
	Now suppose that $\vec{\lambda}_{j-1}^{\phi} = [\vec{\lambda}_{j-1,1}^{\phi}; \dots;\vec{\lambda}_{j-1,m}^{\phi}]$. We want to show that $\vec{\lambda}_{j}^{\phi}$ is an affine function, and also that $\vec{\lambda}_{j}^{\phi} = [\vec{\lambda}_{j,1}^{\phi}; \dots;\vec{\lambda}_{j,m}^{\phi}]$. Let $\vec{\theta}_{j}^{b} = [\vec{\theta}_{j,1}^{b}; \dots;\vec{\theta}_{j,m}^{b}]$. For each $\vec{\theta}_{j,i}^{W}$, let $\vec{\theta}_{j,i}^{W'} = \vec{\theta}_{j,i}^{W} \otimes \vec{e}_{i}$ for $i=1,\dots,m$. Now let, $\vec{\theta}_{j}^{W} = [\vec{\theta}_{j,1}^{W'}; \dots;\vec{\theta}_{j,m}^{W'}]$. It follows that $\vec{\theta}_{j}^{W} \vec{\lambda}_{j-1}^{\phi} = [\vec{\theta}_{j-1,1}^{W} \vec{\lambda}_{j-1,1}^{\phi}; \dots; \vec{\theta}_{j-1,m}^{W} \vec{\lambda}_{j-1,m}^{\phi}]$.
	
	As a result, $\vec{\lambda}_{j}^{\phi}$ is an affine function defined by $\vec{\theta}_{j} = \{\vec{\theta}_{j}^{W}, \vec{\theta}_{j}^{b}\}$. In addition, $\vec{\lambda}_{j}^{\phi} = [\vec{\lambda}_{j,1}^{W}; \dots; \vec{\lambda}_{j,m}^{W}]$ and likewise for $b$. Thus $\phi = [\phi_{1}; \dots; \phi_{m}]$. Since $f_{i} = \phi_{i}$ and $f = [f_{i};\dots;f_{m}]$, it follows that $\phi$ exactly represents $f$. That is $\phi = [f_{i};\dots;f_{m}] = f$. In addition, $\phi$ has depth of $L=\ceil{\log_{2}(n+1)}+1$.
\end{pf}

While this formula gives a bound on the depth for exact representations of PWA on polyhedra functions, it does not give a bound on the size. 



However, the following formula provides lower bound on the maximal number of regions a DNN ReLU with $n_{0}$ inputs, $n_{L}$ outputs, and $L-1$ hidden layers of width $n \geq n_0$ can compute~\cite{montufar2014number}:
\begin{equation}
\label{eq:region_lower_bound}
\left( \prod_{i=1}^{L-1} \left\lfloor \frac{n_{i}}{n_{0}}\right \rfloor^{n_{0}}\right) 
\sum_{j=0}^{n_{0}} \left(
\begin{matrix}
n_{L} \\
j \\ 
\end{matrix} \right).
\end{equation}
These two formulas can be used to aid in the design of the proper neural network architecture for a given problem. For example, if one had \textit{a priori} knowledge of an upper bound on the number of polyhedra regions of the PWA on polyehdra function to be approximated, one could first choose an appropriate depth according to Eqn.~\eqref{eq:network_depth}, and then choose an appropriate layer width according to Eqn.~\eqref{eq:region_lower_bound}.

\subsection{Supervised Learning}

The proposed control law $\pi^{A}_{0}$ first trains a neural network $\phi(\vec{x};\vec{\theta}): \mathbb{R}^{n} \rightarrow \mathbb{R}^{N \cdot (n+m)}$ to approximate $\phi(\vec{x};\vec{\theta}) \approx \pi^{*}$, the optimal open loop mapping. With this approach, the neural network outputs the \textit{sequence} of predicted control inputs and states over the time horizon $N$, rather then just the first control input.

The neural network parameters are optimized using a supervised learning approach that minimizes a loss function based on the Lagrangian. To optimize this loss function, we first generate a dataset $\mathbb{D} = \{\vec{x}_{i},\vec{z}_{i}^{*}, \vec{\lambda}_{i}^{*}, \vec{\nu}_{i}^{*} \}_{i=1}^{N_{D}}$ where $N_{D}$ is the size of the dataset. We assume that we have access to an efficient oracle $\mathbb{O}$, which given a state $\vec{x}$, will output the optimal primal and dual variables $(\vec{z}^{*}, \vec{\lambda}^{*},\vec{\nu}^{*})$. For the convex QP, this oracle can be a primal-dual QP solver.

We use the Sobol Sequence to generate a sequence of data points $\vec{x}$. The Sobol Sequence~\cite{sobol1967distribution} is a Quasi-Monte Carlo (QMC) method which is used in numerical integration due to it's ability to more evenly distribute points across a space compared to random sampling. As a result, it can also be used in the function approximation context when an even distribution of inputs is desired.

\begin{algorithm}[t]
	\caption{Generate Dataset}
	\label{alg:generate_dataset}
	\begin{algorithmic}[1]
		\Procedure{Generate Dataset}{}
		\State $\backslash \backslash N_{S}$ is length of Sobol Sequence
		\State $\backslash \backslash \mathcal{X}_{\textrm{gen}}$ is hypercube
		\State $\backslash \backslash \mathbb{O}$ is a QP Solver (oracle)
		\State Generate $\mathbb{D}_{sobol} = \{ \vec{x}_{i} | \vec{x}_{i} \in \mathcal{X}_{\textrm{gen}} \}|_{i=1}^{N_{S}}$ from Sobol Sequence
		\State $\mathbb{D} = \emptyset$
		\For{$i = 1 \dots N_{S}$}
		\State $(\textrm{feasible}_{i}, \vec{z}^{*}_{i}, \vec{\lambda}^{*}_{i}, \vec{\nu}^{*}_{i}) = \mathcal{O}(x_{i})$
		\If{$\textrm{feasible}_{i} == True$}
		\State $\mathbb{D} = \mathbb{D} \cup (\vec{x}_{i},\vec{z}_{i},\vec{\lambda}_{i},\vec{\nu}_{i})$
		\EndIf
		\EndFor
		\Return{$\mathbb{D}$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

The difficulty with the dataset generation process is that without pre-computing the primal feasible set $\mathcal{X}_{0}$, a given $\vec{x}$ is not known to be feasible until a feasibility problem is solved. An explicit representation of this feasible set $\mathcal{X}_{0}$ can be computationally challenging to acquire, so instead, we use rejection sampling, where we define a hypercube $\mathcal{X}_{\textrm{gen}}$ where $\mathcal{X}_{0} \subseteq \mathcal{X} \subseteq \mathcal{X}_{\textrm{gen}}$. The dataset generation algorithm computes the Sobol Sequence of size $N_{S}>N_{D}$ within $\mathcal{X}_{\textrm{gen}}$, applies the oracle $\mathbb{O}$ on each of these points, and stores the states and corresponding optimal primal dual variables that are feasible. The dataset algorithm is summarized in Alg.~\eqref{alg:generate_dataset}.


After generating dataset $\mathbb{D}$, we then minimize the following empirical loss function over the dataset wrt. the network parameters $\vec{\theta}$:

\begin{equation}
\label{eq:least_squares_Lagrangian}
\sum_{i=1}^{N_{B}}(\mathcal{L}(\phi(\vec{x}_{i};\vec{\theta}), \vec{\lambda}_{i}^{*}, \vec{\nu}_{i}^{*}) - \mathcal{L}(\vec{z}_{i}^{*}, \vec{\lambda}_{i}^{*}, \vec{\nu}_{i}^{*}))^{2}
\end{equation}

Since we are using the optimal dual variables $(\vec{\lambda}_{i}^{*}, \vec{\nu}_{i}^{*})$, by strong duality~\eqref{eq:strong_duality}, the unique minimizer in the primal variable space $\vec{z}$ to~\eqref{eq:least_squares_Lagrangian} are the optimal primal variables $\vec{z}^{*}$. Note that using this loss function is different from the standard supervised learning loss functions such as minimizing the $\ell_{2}$ loss in the primal variable space. A discussion related to the choice of this loss function is provided in Sec.~\ref{sec:loss_functions}.

We use a standard mini-batch optimization approach to train the network by first sampling a mini-batch of size $N_{b}$, computing the loss in~\eqref{eq:least_squares_Lagrangian} except over the mini-batch instead of the entire dataset, and then backpropagating the error to update the neural network parameters $\vec{\theta}$ using a method such as stochastic gradient descent (SGD), or RMSProp~\cite{tieleman2012lecture}. The supervised learning algorithm to train the neural network is performed offline, and is summarized in Alg.~\eqref{alg:training_neural_network}.

\begin{algorithm}[t]
	\caption{Offline Supervised Learning}
	\label{alg:training_neural_network}
	\begin{algorithmic}[1]
		\Procedure{Train Neural Network}{}
		\State $\backslash \backslash \phi$ is the neural network
		\State $\backslash \backslash \theta$ are the network parameters
		\State $\backslash \backslash \mathcal{X}_{\textrm{gen}}$ is a hypercube
		\State $\backslash \backslash \mathcal{O}$ is a QP Solver (oracle)
		\State $\backslash \backslash N_{S}$ is length of Sobol Sequence
		\State $\backslash \backslash N_{B}$ is batch size 
		\State $\mathbb{D} = \textrm{CREATE DATASET}(N_{S},\mathcal{X}_{\textrm{gen}},\mathcal{O})$
		\Repeat
		\State Sample mini-batch $\{x_{i},z^{*}_{i},\lambda^{*}_{i},\nu^{*}_{i}\}|_{i=1}^{N_{B}}$ from $\mathbb{D}$
		\State Compute error gradient $\nabla \theta$ of Eqn.~\eqref{eq:least_squares_Lagrangian}
		\State Update $\theta_{t+1} = \theta_{t} + \nabla \theta$
		\Until{Convergence}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\subsection{Space Filling Tree}
A naive rejection sampling approach for generating the dataset to train the neural network will not scale to high dimensions. The reason is because for many problems, as the dimensionality increases, the volume of the feasible set $\mathcal{X}_{0}$ relative to $\mathcal{X}_{\textrm{gen}}$ will tend to 0. The intuition is similar to the ratio of the volume of a ball inscribed inside a cube. \textcolor{red}{Make these statements more precise}. As a result, we develop a correlated sampling approach that is inspired by the idea of space filling trees. \textcolor{red}{Add citation}. 

The intuition behind our correlated sampling strategy is to start from a feasible point which we call the seed, choose a goal point according to an external method such as random sampling or the Sobol Sequence, and shoot along the ray originating from the feasible point to the goal point. We use a simple line search method to check the feasilibity of each point along the ray starting from the feasible point, and add each intermediate point into our dataset if it is feasible. We terminate once an intermediate point is determined to be infeasible since all succeeding points will also be infeasible since the feasible region is convex.

We then randomly sample a point from our current dataset, set that point as the seed, and repeat. The last step necessary for this strategy is choosing the initial seed point to start from. For all constrained infinite-horizon LQR problems, we know at least one point that lies inside the feasible set, which is the equilibrium point we are trying to stabilize the system around. We assume that this point is the origin, as we can rewrite the linear system to make the equilibrium point the origin. The algorithm for the space filling tree sampling method is described in Alg. \ref{alg:space_filling_tree}.

There are two reasons why this correlated sampling approach is more efficient than naive rejection sampling. The first is that by exploiting the convexity of the feasible region, the majority of the points being tested will be feasible since we can stop checking after the first infeasibility. The second reason is that by using the line search method, we effectively have a good initial guess to hot-start a QP solver at every iteration. By using these hot starts with an appropriate solver, such as an active set solver, we can greatly reduce the number of iterations needed to solve for succeeding points.

\begin{algorithm}[t]
	\caption{Space Filling Tree Sampling Algorithm}
	\label{alg:space_filling_tree}
	\begin{algorithmic}[1]
		\Procedure{Space Filling Tree Sampling}{}
		\State $\backslash \backslash \mathbb{O}$ is an active set QP Solver (oracle)
		\State $\mathbb{D} = \{x_{0}\}$ where $x_{0}$ is the equilibrium point
		\For{$i = 1 \dots N_{S}$}
		\State Sample goal point $g_{i}$
		\State Sample seed point $s_{i} \in 
		\mathbb{D}$
		\State $\backslash \backslash$ Perform line search
		\For{$j=1 \dots N$}
		\State $x_{i,j}$ are the points along the line where $x_{i,0}$ is the seed point, $x_{i,N}$ is the goal point
		\State Hot start $\mathbb{O}$ with $x_{i,j-1}$
		\State $(\textrm{feasible}_{i,j}, \vec{z}^{*}_{i,j}, \vec{\lambda}^{*}_{i,j}, \vec{\nu}^{*}_{i,j}) = \mathbb{O}(x_{i,j})$
		\If{$\textrm{feasible}_{i} == True$}
		\State $\mathbb{D} = \mathbb{D} \cup (\vec{x}_{i,j},\vec{z}_{i,j},\vec{\lambda}_{i,j},\vec{\nu}_{i,j})$
		\EndIf	
		\EndFor
		\EndFor
		\Return{$\mathbb{D}$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\subsection{Active Set}

While the minimization of the Lagrangian loss function~\eqref{eq:lagrangian} during training will penalize constraint violations using optimal dual variables, the trained neural network will still potentially violate constraints since it may not have the capacity to represent the optimal control law, it will not be trained to a global optima, and also it is trained on a dataset of finite size. In addition, even when it outputs feasible primal variables, the resulting sub-optimality gap may be larger than necessary to guarantee asymptotic stability. 

For these reasons, in order to guarantee recursive feasibility and asymptotic stability, we use a \textit{guarantees by construction} approach by introducing a second step to the proposed control law consisting of an active set method where the initial point is provided by the output of the neural network.

Active set methods solve a sequence of equality-constrained quadratic subproblems. The goal of these methods is to predict the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*}; \vec{x})$ where a constraint $i \in \mathcal \mathcal{W}_{\mathcal{A}}(\vec{z}^{*}; \vec{x})$ indicates that that constraint is tight, or satisfied with equality, at the optimal solution. It is clear that all equality constraints must be in the optimal active set, otherwise the active set corresponds to a region that does not contain primal feasible points. Thus the goal of the active set method is to identify which of the inequality constraints will be active at the optimal solution. 

\begin{algorithm}[t]
	\caption{Active Set}
	\label{alg:active_set}
	\begin{algorithmic}[1]
		\Procedure{Active Set}{}
		\State $\backslash \backslash \vec{z}^{init}$ is the initial guess
		\State $\backslash \backslash \gamma(\vec{x})$ is desired sub-optimality level
		\State $\backslash \backslash~Phase~1$
		\State Compute feasible $\vec{z}^{0}$ from $\vec{z}^{init}$ by solving Phase 1 problem~\eqref{eq:linear_feasibility_problem}
		\State Set $\mathcal{W}^{0}$ to be a linearly independent subset of active constraints at $\vec{z}_{0}$
		\State $\backslash \backslash~Phase~2$
		\For{k=0,1,2,\dots}
		\State Solve Eqn.~\eqref{eq:active_set_subproblem} to find $\vec{p}^{k}$
		\If{($\vec{p}^{k} = 0$)}
		\State Compute Lagrange multiplier $\vec{\lambda}^{k}$ and $\vec{\nu}^{k}$
		\If{$\lambda^{k,i} \geq 0~\forall~i \in \mathcal{W}^{k} \cap \mathcal{I}$}
		\State \Return{$\vec{z}^{k}$}
		\Else 
		\State Compute feasible duality gap $\eta(\vec{z}^{k},\vec{\lambda}^{k},\vec{\nu}^{k};\vec{x})$
		\If{$\eta(\vec{z}^{k},\vec{\lambda}^{k},\vec{\nu}^{k};\vec{x})<\gamma(\vec{x})$}
		\State \Return{$\vec{z}^{k}$}
		\Else
		\State Set $i = \argmin_{i \in \mathcal{W}^{k} \cap 	\mathcal{I}} \lambda^{k,i}$
		\State $\vec{z}^{k+1} = \vec{z}^{k}$; $\mathcal{W}^{k+1} = \mathcal{W}^{k} \setminus \{i\}$
		\EndIf
		\EndIf
		\Else{~($\vec{p}^{k} \neq 0$)}
		\State Compute $\alpha^{k}$ from Eqn.~\eqref{eq:step_length}
		\State $\vec{z}^{k+1} = \vec{z}^{k} + \alpha^{k}\vec{p}^{k}$
		\If{there are blocking constraints}
		\State Add blocking constraint to $\mathcal{W}^{k}$ to get $\mathcal{W}^{k+1}$
		\Else
		\State $\mathcal{W}^{k+1} = \mathcal{W}^{k}$
		\EndIf
		\EndIf
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

The proposed control law $\pi_{0}^{A}$ uses the active set method since it is well suited to \textit{warm-starts}~\cite{wright1999numerical}. Thus a good initial guess, such as the neural network output $\vec{z}_{init} = \phi(\vec{x};\vec{\theta})$, can greatly speed up the optimization method. For example, if we know the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*};\vec{x})$, then we can obtain the optimal primal variables $\vec{z}^{*}$ by solving the following equality constrained sub-problem:

\small
\begin{equation}
\label{eq:optimal_active_set_subproblem}
\begin{aligned}
& \underset{\vec{z}}{\text{argmin}}  
& & \vec{z}^{T}\mat{H}\vec{z} \\
& \text{s.t.}
& & \vec{g}^{(i)}_{0,\textrm{in}}\vec{z} = \vec{h}^{(i)}, \qquad i \in \mathcal{W}_{\mathcal{A}}(\vec{z}^{*};\vec{x})\\
& & & \vec{g}^{(i)}_{0,\textrm{eq}}\vec{z} = \vec{h}^{(i)}.\\
\end{aligned}
\end{equation}
\normalsize
However, we do not necessarily know the optimal active set $\mathcal{W}_{\mathcal{A}}(\vec{z}^{*},\vec{x})$ beforehand, but instead can obtain a good guess from the neural network output $\phi(\vec{x};\vec{\theta})$ by identifying a linearly independent subset of constraints $\mathcal{W}_{0}$ that are active at a feasible point $\vec{z}^{0}$ that is close to $\vec{z}^{init} = \phi(\vec{x};\vec{\theta})$. The active set method will take a desired sub-optimality level $\gamma(\vec{x})$, update $\vec{z}^{init}$ and $\mathcal{W}_{0}$ while maintaining primal feasibility until it finds a $\vec{z}^{k}$ which satisfies $\sigma(\vec{z}^{k};\vec{x}) \leq \gamma(\vec{x})$.

Active set methods consist of two phases and is summarized in Alg.~\eqref{alg:active_set}. The \textit{Phase 1} method finds an initial feasible point $\vec{z}^{0}$ from the network output $\vec{z}^{init}$, and the \textit{Phase 2} method takes $\vec{z}^{0}$ and iterates $k = 1,\dots$ until $\sigma(\vec{z}^{k};\vec{x}) \leq \gamma(\vec{x})$ is achieved. A $\vec{z}^{init}$ close to $\vec{z}^{*}$ warm starts the active set method and significantly reduces the computation load by both the \textit{Phase 1} and \textit{Phase 2} methods.

Given the neural network output $\vec{\phi}(\vec{x};\vec{\theta})$, the Phase 1 method corresponds to solving the following linear feasibility problem:

\small
\begin{equation}
\label{eq:linear_feasibility_problem}
\begin{aligned}
& \underset{(\vec{z}, \vec{y})}{\text{argmin}}  
& & \vec{e}^{T}\vec{y} \\
& \text{s.t.}
& & \vec{g}^{(i)}_{0,\textrm{eq}}\vec{z} + \vec{\gamma}^{(i)}y^{(i)} = \vec{h}^{(i)}_{0,\textrm{eq}}, \qquad i \in \mathcal{E}\\
& & & \vec{g}^{(i)}_{0,\textrm{in}}\vec{z} + \vec{\gamma}^{(i)}y^{(i)} \leq \vec{h}^{(i)}_{0,\textrm{in}}, \qquad i \in \mathcal{I}\\
& & & \vec{y} \geq 0
\end{aligned}
\end{equation}
\normalsize

where $e = (1, \dots, 1)^{T}$, $\gamma^{(i)} = -\textrm{sign}(\vec{g}^{(i)}_{0,\textrm{eq}}\vec{z^{init}} - \vec{h}^{(i)}_{0,\textrm{eq}})$ for $i \in \mathcal{E}$, and $\gamma^{(i)} = -1$ for $i \in \mathcal{I}$. A feasible initial point for this problem is $\vec{z}^{init}$, $y^{(i)} = |\vec{g}^{(i)}_{0,\textrm{eq}}\vec{z}^{init} - h^{(i)}_{0,\textrm{eq}}|$ for $i \in \mathcal{E}$, and $y^{(i)} = \max(\vec{g}^{(i)}_{0,\textrm{in}}\vec{z}^{init} + \vec{\gamma}^{(i)}y^{(i)} - \vec{h}^{(i)}_{0,\textrm{in}}, 0)$ for $i \in \mathcal{I}$. 

If $\vec{z}^{init}$ is primal feasible, then $(\vec{z}^{init}, \vec{0})$ is optimal for Problem~\eqref{eq:linear_feasibility_problem}. In addition, if Problem~\eqref{eq:decoupled_batch_problem} has a feasible solution, then the optimal objective function for Problem~\eqref{eq:linear_feasibility_problem} is $0$, and any solution yields a feasible point for Problem~\eqref{eq:decoupled_batch_problem}. 

Once a solution to Problem~\eqref{eq:linear_feasibility_problem} is found, the initial primal feasible point $\vec{z}^{0}$ can be extracted. The \textit{Phase 2} method iterates until a desired sub-optimality level $\epsilon$ is achieved. The Phase 2 method computes an initial working set $\mathcal{W}^{0}$ consisting of a linearly independent subset of the active constraints at $\vec{z}^{0}$. It then iteratively computes a step direction $\vec{p}^{k}$ and updates $\mathcal{W}^{k}$ by either adding or removing constraints while maintaining primal feasibility of each iterate $\vec{z}^{0}$. It terminates when $\sigma(\vec{z}^{k};\vec{x}) \leq \gamma(\vec{x})$.

The step direction $\vec{p}^{k}$ is computed as follows. Define $\vec{p} = \vec{z} - \vec{z}^{k}$, and $\vec{g}^{k} = \mat{H}\vec{z}^{k}$. By substituting into the objective function of Problem~\eqref{eq:decoupled_batch_problem} and dropping the constant $\vec{x}^{T}\mat{Q}\vec{x}$ term, we get that 

\begin{equation}
\label{eq:active_step_step_objective}
\begin{aligned}
J_{0}(\vec{x},\vec{z}) &= \vec{z}^{T}\mat{H}\vec{z} \\
&= (\vec{z}^{k} + \vec{p})^{T}\mat{H}(\vec{z}^{k}+\vec{p}) \\
&= [\vec{z}^{k}]^{T}\mat{H}\vec{z}^{k} + 2[\vec{z}^{k}]^{T}\mat{H}\vec{p} + \vec{p}^{T}\mat{H}\vec{p} \\ 
&= \vec{p}^{T}\mat{H}\vec{p} + 2[\mat{H}\vec{z}_{k}]^{T}\vec{p} + c
\end{aligned}
\end{equation}
where $c = \vec{z}_{k}^{T}\mat{H}\vec{z}_{k}$ is a constant that does not depend on $p$. Thus by setting the constraints in $\mathcal{W}^{k}$ to equality and temporarily ignoring all other constraints, we can solve the equality-constrained sub-problem:

\small
\begin{equation}
\label{eq:active_set_subproblem}
\begin{aligned}
& \underset{\vec{p}}{\text{argmin}}  
& & \vec{p}^{T}\mat{H}\vec{p} + 2[\mat{H}\vec{z}_{k}]^{T}\vec{p} \\
& \text{s.t.}
& & \vec{g}^{(i)}_{0,\textrm{in}}\vec{p} = 0, \qquad i \in \mathcal{W}_{k}\\
& & & \vec{g}^{(i)}_{0,\textrm{eq}}\vec{p} = 0,\\
\end{aligned}
\end{equation}
\normalsize

of which the solution is denoted as $\vec{p}^{k}$. Since $\vec{g}^{(i)}_{0,(\cdot)}\vec{p}=0$, for each constraint $i \in \mathcal{W}^{k}$, it follows that if the constraint $\vec{g}^{(i)}_{0,(\cdot)}\vec{z}_{k} = \vec{h}^{(i)}$ were satisfied at iteration $k$, then the constraint will also be satisfied at iteration $k+1$. If the optimal $\vec{p}^{k}$ is non-zero, we have to decide a step length $\alpha^{k}$ so that $\vec{z}^{k} + \alpha^{k} \vec{p}^{k}$ is still feasible for all constraints. This block constraint can only be an inequality constraint. Thus we only have to worry about the inequality constraints where $\vec{g}^{(i)}_{0,\textrm{in}}\vec{p}^{k} > 0$, thus we compute a step-length 

\begin{equation}
\label{eq:step_length}
\alpha^{k} = \min \left(1, \min_{i \neq \mathcal{W}_{k}, \vec{g}^{(i)}_{0,\textrm{in}}\vec{p}_{k}>0}\frac{h^{(i)}-\vec{g}^{(i)}_{0,\textrm{in}}\vec{z}^{k}}{\vec{g}^{(i)}_{0,\textrm{in}}\vec{p}^{k}} \right)
\end{equation}

and set $\vec{z}^{k+1} = \vec{z}^{k} + \alpha^{k}\vec{p}^{k}$. If $\alpha^{k} < 1$, then the the step along $\vec{p}^{k}$ was blocked by some inequality constraint, and that constraint is added to $\mathcal{W}^{k}$ create a new working set $\mathcal{W}^{k+1}$.

These iterations are continued until a point $\vec{z}^{k}$ is reached that minimizes the quadratic objective over the current working set $\mathcal{W}^{k}$. This can be identified because Problem~\eqref{eq:active_set_subproblem} will have a solution $\vec{p} = 0$. When this occurs, we check if $\sigma(\vec{z}^{k}) < \gamma(\vec{x})$. If it is, we return $\vec{z}^{k}$, otherwise, we inspect the inequality Lagrange multipliers $\vec{\lambda}^{k}$ in our current working set $\mathcal{W}^{k}$. One of the $\lambda^{k,i} < 0$, otherwise the $\vec{z}^{k}$ would have been the optimal solution. We find the constraint $i$ with the most negative $\lambda^{k,i}$ and drop it from the working set $\mathcal{W}^{k}$ to get a new working set $\mathcal{W}^{k+1}$ and continue iterating.

Iterating this fashion will terminate in a finite number of steps~\cite{wright1999numerical} and return a primal $\vec{z}^{k}$ that is both primal feasible and satisfy $\sigma(\vec{z}^{k}; \vec{x}) \leq \gamma(\vec{x})$. 

\subsection{Proposed Control Law}
Combining the neural network and active set components will result in feasible $\gamma$-optimal open loop mapping $\pi^{A}(\vec{x})$. Applying it in a receding horizon fashion will yield the approximate RHC $\pi_{0}^{A}(\vec{x})$, which by Thm.~\ref{thm:approximate_RHC_stability} is recursively feasible and asymptotically stable. The proposed control law $\pi_{0}^{A}(\vec{x})$ is described in Alg.~\ref{alg:proposed_control_law}.

\begin{algorithm}[t]
	\caption{Proposed Control Law}
	\label{alg:proposed_control_law}
	\begin{algorithmic}[1]
		\Procedure{Sub-Optimal Control Law}{$\tilde{\pi}$, $\vec{x}$, $\mat{M}$}
		\State $\backslash \backslash~ \phi(\vec{x};\vec{\theta})$ is the neural network
		\State $\backslash \backslash~ \vec{x}$ is the current state
		\State $\backslash \backslash~ \mat{M}$ is matrix defining contribution to the stage cost dependent on the state
		\State $\gamma(\vec{x}) = \vec{x}^{T}\mat{M}\vec{x}$
		\State $\vec{z}^{init} = \phi(\vec{x};\vec{\theta})$ \Comment{Call Neural Network}
		\State Obtain $\vec{z}^{A}$ by calling Alg.~\ref{alg:active_set} with $\vec{z}_{init}$ and $\gamma(\vec{x})$
		\State Implement the first control action $u_{0}^{A}$ in $\vec{z}^{A}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}





==> tex/Results.tex <==
\section{Results}
\begin{figure*}[t!]
\begin{center} 
 \setlength\extrarowheight{5pt}
 \resizebox{\textwidth}{!}
 {\begin{tabular}{||c | c| c| c ||} 
 \hline
 Measure & Feasible Control Law (Analytic Center) & Predicted Control Law (No Projection) & Final Control Law\\ [0.6ex] 
 \hline\hline
 Average Value Error & 91.4 (27.1 $\%$) & 0.16 (0.44 $\%$) & 2.58 (0.55 $\%$) \\
 \hline\hline
 Median Value Error & 91.8 (26.6 $\%$) & 0.10 (0.03 $\%$) & 0.12 (0.03 $\%$) \\
  \hline\hline
  Maximum Value Error & 83.9 $\%$ & 1.8 $\%$ & 31.5 $\%$ \\
  \hline\hline
 Number Find Feasible (29,970) & 25,122 (83.8 $\%$) & 24,881 (83.0 $\%$) & 27,456 (91.6 $\%$) \\
    \hline\hline
 Number $< 3\%$ error  & 0.0 $\%$  & 100 $\%$ & 94.4 $\%$ \\
    \hline\hline
\end{tabular}}
\end{center}
\caption{Results }
\label{fig:oscillating_masses}
\end{figure*}


\begin{figure*}[t!]
\begin{center} 
 \setlength\extrarowheight{5pt}
 \resizebox{\textwidth}{!}
 {\begin{tabular}{||c | c | c |c |c |c ||} 
 \hline
 Margin & Lagrangian Train {\tiny ($\# 451,266$)} & $\ell_{2}$ Train {\tiny ($\# 451,266$)} & Lagrangian Test {\tiny ($\# 29,868$)} & $\ell_{2}$ Test {\tiny ($\# 29,868$)} & No Dropout Test {\tiny ($\# 29,868$)} \\ [0.6ex] 
 \hline\hline
 0.00 & $0.0 \%$ {\tiny ($1$)}  & $0.0 \%$ {\tiny ($7$)}  & $0.0 \%$ {\tiny ($0$)}& $0.0 \%$ {\tiny ($0$)} & $0.0 \%$ {\tiny ($1$)}\\
 \hline\hline
 0.01 & $83.1 \%$ {\tiny ($375,120$)} & $82.1 \%$ {\tiny ($370,433$)}  & $83.5 \%$ {\tiny ($24,932$)} & $82.4 \%$ {\tiny ($24,621$)} & $85.0 \%$ {\tiny ($25,400$)} \\
  \hline\hline
  0.05 &  $88.1 \%$ {\tiny ($397,932$)} & $86.3 \%$ {\tiny ($389,625$)}  & $88.2 \%$ {\tiny ($26,367$)} & $86.6 \%$ {\tiny ($25,876$)} & $91.6 \%$ {\tiny ($27,362$)}\\
  \hline\hline
 0.10 &  $93.7 \%$ {\tiny ($422,904$)} & $90.9 \%$ {\tiny ($410,225$)} & $93.4 \%$ {\tiny ($27,905$)} & $90.9 \%$ {\tiny ($27,162$)} & $96.1 \%$ {\tiny ($28,715$)}\\
    \hline\hline
 0.15  &  $96.5 \%$ {\tiny ($435,523$)} & $94.3 \%$ {\tiny ($425,361$)} & $96.2 \%$ {\tiny ($28,745$)}  & $94.1 \%$ {\tiny ($28,131$)} & $98.1 \%$ {\tiny ($29,320$)}\\
    \hline\hline
 0.20  &  $98.1 \%$ {\tiny ($442,772$)}  &  $96.4 \%$ {\tiny ($435,201$)}  & $97.9 \%$ {\tiny ($29,235$)} & $96.4 \%$ {\tiny ($28,786$)} & $99.2 \%$ {\tiny ($29,636$)}\\
    \hline\hline
 0.25 &  $99.1 \%$ {\tiny ($447,347$)} & $97.9 \%$ {\tiny ($441,682$)} & $98.9 \%$ {\tiny ($29,536$)}  & $97.8 \%$ {\tiny ($29,225$)} & $99.7 \%$ {\tiny ($29,783$)} \\
    \hline\hline
 0.50  &  $100.0 \%$ {\tiny ($451,256$)}  &  $99.9 \%$ {\tiny ($450,909$)}     & $100.0 \%$ {\tiny ($29,867$)}& $99.9 \%$ {\tiny ($29,845$)} & $100.0\%$ {\tiny ($29,868$)}\\
    \hline\hline
 1.00  &  $100.0 \%$ {\tiny ($451,266$)} &  $100.0 \%$ {\tiny ($451,266$)}  & $100.0 \%$ {\tiny ($29,868$)} & $100.0 \%$ {\tiny ($29,868$)} & $100.0 \%$ {\tiny ($29,868$)}\\
    \hline\hline
\end{tabular}}
\end{center}
\caption{Percentage Feasible }
\label{fig:oscillating_masses}
\end{figure*}

\begin{figure*}[t!]
\begin{center} 
 \setlength\extrarowheight{5pt}
 \resizebox{\textwidth}{!}
 {\begin{tabular}{||c | c| c| c | c |c | c||} 
 \hline
 Measure & Lagrangian Train  & $\ell_{2}$ Train  & Lagrangian Test& $\ell_{2}$ Test & No dropout Test & Projected\\ [0.6ex] 
 \hline
 Average $\ell_{2}$ error (\textit{primal}) & 0.12 & 0.186 & 0.128  & 0.186 & 0.065 & 0.036\\
 \hline
 Median $\ell_{2}$ error (\textit{primal}) & 0.07 & 0.106 & 0.069  & 0.107 & 0.024 & 0.020 \\
  \hline
  Maximum $\ell_{2}$ error (\textit{primal}) & 8.52 & 11.84 & 4.35 & 6.16 & 4.42 & 1.45\\
  \hline\hline
   Average Value Error (\textit{cond. $< 0.01$ margin}) & 0.70 (0.18$\%$) & 1.58 (0.42$\%$) & 0.72 (0.19$\%$) & 1.58 (0.42$\%$) & 1.76 (0.46$\%$) & 1.16 (0.27$\%$)\\
   \hline
   Median Value Error (\textit{cond. $< 0.01$ margin}) & 0.48 (0.14 $\%$) & 1.32 (0.38 $\%$) & 0.48 (0.14 $\%$) & 1.33 (0.39 $\%$) & 1.36 (0.40 $\%$) & 0.70 (0.19 $\%$)\\
   \hline
   Max Value Error (\textit{cond. $< 0.01$ margin}) & 22.1 (5.1 $\%$) & 32.48 (4.3 $\%$) & 25.6 (5.7 $\%$) & 13.8 (2.6 $\%$) & 23.4 (5.6 $\%$) & 36.4 (5.4 $\%$)\\
   \hline
   Min Value Error (\textit{cond. $< 0.01$ margin}) & -29.4 (-6.6 $\%$) & -26.9 (-6.2$\%$) & -12.0 (-2.6$\%$) & -9.4 (-2.1$\%$) & -10.0 (-2,2$\%$) & 0.02 (0.0$\%$) \\
   \hline\hline
   Average Lagrangian Error (\textit{all}) & 0.58 (0.16 $\%$) & 0.64 (0.17 $\%$) & 0.61 (0.16 $\%$) & 0.65 (0.16 $\%$) & 0.22 (0.05 $\%$) & 0.11 (0.0 $\%$)\\
   \hline
   Median Lagrangian Error (\textit{all}) & 0.37 (0.12 $\%$) & 0.33 (0.11 $\%$) & 0.37 (0.12 $\%$) & 0.33 (0.11 $\%$) & 0.07 (0.02 $\%$) & 0.05 (0.01 $\%$)\\
   \hline
   Max Lagrangian Error (\textit{all}) & 51.3 ( 10.4 $\%$) & 77.0 (15.6 $\%$) & 25.7 (5.9 $\%$) & 41.4 (6.7 $\%$) & 21.06 (5.3 $\%$) & 7.32 (1.9 $\%$)\\
   \hline
   Min Lagrangian Error (\textit{all}) & 0.05 (0.0 $\%$) & 0.05 (0.0 $\%$) & 0.05 (0.0 $\%$) & 0.06 (0.0 $\%$) & 0.01 (0.0 $\%$) & 0.01 (0.0 $\%$)\\
  \hline\hline
\end{tabular}}
\end{center}
\caption{Results statistics }
\label{fig:oscillating_masses}
\end{figure*}

==> tex/Suboptimality.tex <==
\section{Measuring Sub-optimality}

Once the network has be trained, the combination of calling the network and performing the operation to ensure feasibility defines a sub-optimal controller for Problem~\eqref{eq:time_invariant_finite_horizon_problem}. As a result, we would like to know how sub-optimal this approximation is in order to determine whether the network output should be followed or not. Since the neural network is a non-convex function where the outputs have a complicated relationship with the inputs, it is challenging to guarantee a specific level of sub-optimality for all possible states $\vec{x}(t)$. We instead present a method that, for each states $\vec{x}(t)$, uses the \textit{duality gap} from convex optimization theory to provide bounds on the sub-optimality of the neural network prediction.

We define the Lagrangian $\mathcal{L}(\vec{U}_{0}, \vec{\lambda}; \vec{x}(t))$ for Problem~\eqref{eq:coupled_batch_problem} as:

\begin{equation}
\label{eq:Lagrangian}
\begin{aligned}
\mathcal{L}(\vec{U}_{0}, \vec{\lambda}; \vec{x}(t)) &= \vec{U}_{0}^{T}\mat{H}\vec{U}_{0} + 2\vec{x}^{T}(t)\mat{F}\vec{U}_{0} + \vec{x}^{T}(t)\mat{Y}\vec{x}(t) \\
& \qquad + \vec{\lambda}^{T} \left( \mat{G}_{0}\vec{U}_{0} - \vec{w}_{0} - \mat{E}_{0}\vec{x}(t) \right)
\end{aligned}
\end{equation}

The variables $\vec{U}_{0}$ is the primal variable, $\vec{\lambda}$ the dual variables corresponding the inequality constraints, and $\vec{x}(t)$ is the parameter of the problem. Notice that since we are looking at the Lagrangian of the coupled batch problem, there are no equality constraints. To derive the dual cost, we take the partial derivative to find the minimum.

The partial derivative is given by:
\begin{equation}
\begin{aligned}
\frac{\partial \mathcal{L}(\vec{U}_{0}, \vec{\lambda}; \vec{x}(t))}{\partial \vec{U}_{0}} &= 2\mat{H}\vec{U}_{0} + 2\mat{F}^{T}\vec{x}(t) + \mat{G}_{0}^{T}\vec{\lambda} \equiv 0 \\
&\Rightarrow \vec{U}_{0}^{\lambda} = -\mat{H}^{-1} \left( \mat{F}^{T}\vec{x}(t) + \frac{1}{2}\mat{G}_{0}^{T}\vec{\lambda} \right)
\end{aligned}
\end{equation}
The dual cost $g(\vec{\lambda}; \vec{x}(t))$ is thus obtained by plugging in $\vec{U}_{0}^{\lambda}$ into Eqn.~\eqref{eq:Lagrangian}. The dual cost yields a lower bound on the optimal cost $J_{0,c}^{*}(\vec{x}(t))$, which is known as \textit{weak duality}. That is, for any $\lambda \succeq 0$, $g(\vec{\lambda}; \vec{x}(t)) \leq J_{0,c}^{*}(\vec{x}(t))$. More importantly, since Problem~\eqref{eq:coupled_batch_problem} is convex, and if we assume that there exists a $\mat{U}_{0} \in \textrm{\textbf{relint}}~\mathcal{F}_{0}$, Slater's condition holds, so \textit{strong duality} holds for our problem. That is, for each state $\vec{x}(t)$, there exists an optimal dual variable $\vec{\lambda}^{*} \succeq 0$ such that $g(\vec{\lambda}^{*}; \vec{x}(t)) \leq J_{0,c}^{*}(\vec{x}(t))$.

The key idea to obtaining bounds on the sub-optimality of our neural network controller is to utilize these duality gap measures. Given the neural network output for a state $\vec{x}(t)$, followed by the central path projection, we obtain a primal feasible $\hat{\vec{U}}_{0}$. Given these primal variables, we will obtain a candidate dual feasible variable $\hat{\vec{\lambda}}$ by using the \textit{Karush-Kuhn-Tucker (KKT)} optimality conditions.

Let $\prl{\mat{G}_{0}\vec{U}_{0} - \vec{w}_{0} - \mat{E}_{0}x(t)}^{(i)}$ denote the $i$-th row of $\prl{\mat{G}_{0}\vec{U}_{0} - \vec{w}_{0} - \mat{E}_{0}x(t)}$ where $i=1 \dots m_{0}$. The KKT conditions are:

\begin{subequations}

\begin{align}
2\mat{H}\vec{U}_{0} + 2\mat{F}^{T}\vec{x}(t) + \mat{G}_{0}^{T}\vec{\lambda} &= 0 \label{eq:KKT_conditions_stationarity} \\
\prl{\mat{G}_{0}\vec{U}_{0} - \vec{w}_{0} - \mat{E}_{0}x(t)} &\preceq 0 \label{eq:KKT_conditions_primal_feasible}\\
\lambda_{i}\prl{\mat{G}_{0}\vec{U}_{0} - \vec{w}_{0} - \mat{E}_{0}x(t)}^{(i)} &= 0, ~i=1,\dots,m_{0} \label{eq:KKT_conditions_complementary_slackness}\\
\lambda &\succeq 0 \label{eq:KKT_conditions_dual_feasible},
\end{align}
\end{subequations}
where Eqn.~\eqref{eq:KKT_conditions_stationarity} is known as the stationarity condition, Eqn.~\eqref{eq:KKT_conditions_primal_feasible} is the primal feasibility condition, Eqn.~\eqref{eq:KKT_conditions_complementary_slackness} is the complementary slackness condition, and Eqn.~\eqref{eq:KKT_conditions_dual_feasible} is the dual feasibility condition. Since the Problem~\eqref{eq:time_invariant_finite_horizon_problem} is convex, the KKT conditions are necessary and sufficient conditions for an optimal primal-dual pair $(\mat{U}_{0}^{*}, \vec{\lambda}^{*})$.

If we have the optimal primal feasible point $\vec{U}_{0}^{*}$, then we can use the KKT conditions to easily compute an optimal dual feasible point $\vec{\lambda}^{*}$. We can first use the complementary slackness condition~\eqref{eq:KKT_conditions_complementary_slackness} to determine which constraints are active, and thus which $\lambda_{i}$ is positive. Let $\mathcal{A}^{*}(\vec{x}(t)) = \{i~|~\prl{\mat{G}_{0}\vec{U}_{0}^{*} - w_{0} - \mat{E}_{0}\vec{x}(t)}^{(i)} = 0\}$ denote the set of active constraints for the optimal $\vec{U}_{0}^{*}$, and $\mathcal{NA}^{*}(\vec{x}(t)) = \{i~|~\prl{\mat{G}_{0}\vec{U}_{0}^{*} - w_{0} - \mat{E}_{0}\vec{x}(t)}^{(i)} < 0\}$ the set of inactive constraints. By the complementary slackness condition, for any $i \in \mathcal{NA}$, $\lambda_{i}=0$. As a result, by using the optimal primal feasible point, we can compute the values for all $\lambda_{i}$ that correspond to inactive constraints.

We are left with the dual variables $\lambda_{i}$ such that $i \in \mathcal{A}^{*}(\vec{x}(t))$. The dual feasibility condition requires that each $\lambda_{i} > 0$, and the stationarity condition provides a way to compute the correct $\lambda_{i}^{*}$ given the primal variables. 

The difficulty occurs when we do not have the optimal feasible points $\vec{U}_{0}^{*}$, but rather a sub-optimal approximation given by our neural network $\hat{\vec{U}}_{0}^{*}$. Since this point is not optimal, there will not be a corresponding $\lambda$ that will perfectly satisfy all of the KKT conditions. However, weak duality implies that any dual feasible point will provide a lower bound to $J_{0,c}^{*}$, and we just need to heuristically choose a $\lambda$ that minimizes this bound. 

As a result, we can use the same method as for the optimal primal feasible point, as a heuristic to choose a dual feasible $\lambda$, and use the resulting dual cost as our bound. The central path projection ensures that our primal feasible point $\hat{\vec{U}}_{0}^{*}$ satisfies the primal feasibility condition~\eqref{eq:KKT_conditions_primal_feasible}. We can define the active set $\hat{\mathcal{A}}^{*}(\vec{x}(t)) = \{i~|~\prl{\mat{G}_{0}\hat{\vec{U}}_{0}^{*} - w_{0} - \mat{E}_{0}\vec{x}(t)}^{(i)} \geq -\epsilon\}$ for some $\epsilon > 0$ threshold chosen by the user, as well as the inactive set $\widehat{\mathcal{NA}}^{*}(\vec{x}(t)) = \{i~|~\prl{\mat{G}_{0}\hat{\vec{U}}_{0}^{*} - w_{0} - \mat{E}_{0}\vec{x}(t)}^{(i)} < -\epsilon\}$. We can similarly use the complementary slackness condition to set all $\hat{\lambda}^{*}_{i} = 0$ for $i \in \widehat{\mathcal{NA}}$. Now we can perform a non-negative least squares regression (NNLS) to find the remaining dual variables:

\small
\begin{equation}
\label{eq:non_negative_least_squraes}
\begin{aligned}
& \underset{\hat{\vec{\lambda}}}{\text{argmin}}  
& & \frac{1}{2} || 2\mat{H}\vec{U}_{0} + 2\mat{F}^{T}\vec{x}(t) - \mat{G}_{0}^{T}\vec{\lambda}||_{2}^{2} \\
& \text{s.t.}
& & \hat{\lambda}_{i} > 0, ~i \in \widehat{\mathcal{NA}}^{*}(\vec{x}(t)) \\
& & & \hat{\lambda}_{i} = 0, ~i \in \widehat{\mathcal{A}}^{*}(\vec{x}(t)) \\
\end{aligned}
\end{equation}
\normalsize

Solving this NNLS problem has lower computational complexity than the original problem because we have eliminated many of the dual variables through the complementary slackness condition. In addition, while calling the network and performing the central path projection needs to be executed in real-time, this NNLS operation only needs to be performed when the quality of the neural network trajectory needs to be verified. This can happen at a slower frequency, since it is not necessarily needed to execute the controller.

Thus, given our neural network primal feasible point $\hat{\vec{U}}_{0}^{*}$, we can compute a dual feasible points $\hat{\vec{\lambda}}$. By computing the primal cost $\hat{J}_{0,c}^{*}(\vec{x}(t))$ corresponding to $\hat{\vec{U}}_{0}^{*}$, as well as the dual cost $\hat{g}$ corresponding to $\hat{\vec{\lambda}}$, we can compute the duality gap $\hat{\mathcal{G}} = \hat{J}_{0,c}(\vec{x}(t)) - \hat{g} \geq 0$. Since $\hat{J}_{0,c}(\vec{x}(t)) \geq J_{0,c}^{*}(\vec{x}(t))$, and $\hat{g} \leq J_{0,c}^{*}(\vec{x}(t))$, $\hat{\mathcal{G}}$ provides an upper bound on the sub-optimality of the neural network controller $\hat{J}_{0,c}(\vec{x}(t)) - J_{0,c}^{*}(\vec{x}(t))$ starting at state $\vec{x}(t)$.



==> tex/TechnicalApproach.tex <==
\section{Technical Approach and Overview}

Our primary motivation is learning a controller with guarantees for high-dimensional problems with large state and input dimensions and long time horizons. Large problems are challenging since traditional explicit MPC approaches become too computationally expensive, and even implicit MPC may require custom architectures on FPGAs for real-time inference~\cite{jerez2014embedded}. We propose a hybrid explicit-implicit procedure that merges an offline trained neural network with an online primal active set solver to compute a planner $\pi$. The neural network approximation of the planner enables our procedure to scale to these large problems. The primal active set solver then provides a few corrective steps to meet the conditions necessary to guarantee recursive feasibility and asymptotic stability.

In Sec.~\ref{sec:neural_network}, we describe the offline neural network architecture training procedure. The neural network approximates a planner $\tilde{\pi}$ by mapping the state $\vec{x}$ to a primal prediction $\tilde{\vec{z}}$. We highlight the connections between neural networks with rectified linear unit (ReLu) activation functions and the optimal planner and RHC for MPC problems. We then introduce a primal-dual loss function based on the Lagrangian function to train the neural network. 

In Sec.~\ref{sec:guarantees_certificates}, we describe the conditions necessary to obtain guarantees of recursive feasibility and asymptotic stability of the RHC $\mu$ corresponding to an optimal and suboptimal planner $\pi$. These conditions center on both checking for primal feasibility and bounding the sub-optimality of the planner. We then introduce a procedure to obtain certificates of primal feasibility and sub-optimality for a given state parameter $\vec{x}$ and the primal variable $\vec{z}$, without the need of additional inputs such as the dual variables $\vec{\nu},\vec{\lambda}$.

In Sec.~\ref{sec:active_set}, we introduce primal active set methods. We describe how to merge these methods with the neural network in a manner that reduces the extra necessary online computation. The combination computes a new suboptimal planner $\hat{\pi}$ that yields a RHC $\hat{\mu}$ that is recursively feasible and asymptotically stable.

In Sec.~\ref{sec:space_filling}, we highlight the practical issues that arise when scaling the proposed procedure to high dimensional problems. The main challenge is drawing samples from the domain of our planner $\mathcal{X}_{0}$ to train and evaluate the neural network, as $\mathcal{X}_{0}$ is difficult to compute for large problems. Instead we have a \textit{membership oracle} in the form of a QP solver that given a state parameter $\vec{x}$, will determine whether the corresponding QP~\eqref{eq:decoupled_batch_problem} has a solution. We demonstrate how standard sampling methods such as gridding or Monte Carlo rejection sampling will not scale to high dimensions, and introduce the theory of \textit{geometric random walks} to surpass this problem. We then develop a practical method motivated by this theory to generate large datasets for large scale problems. 

In Sec.~\ref{sec:results}, we present results and analysis on four systems that demonstrate the ability of our proposed approach to scale to large systems. We also provide illustrative metrics that highlight the encountered challenges that shaped the development of this method. The largest problem we analyze has $36$ states, $9$ inputs, and time horizon of $50$, and our results indicate that our method can be applied to even larger systems. We did not analyze a larger system since the implementation we used to generate Sobol sequences (described in Sec.~\ref{sec:space_filling}) was limited to $40$ dimensions.


==> tex/rlExamples.tex <==
\section{Reinforcement Learning Examples}



%============ Pendulum ==============================%
\subsection{Pendulum}
We consider an inverted pendulum system with state $x = (\theta, \dot{\theta})^T$ where $\theta$ is the angle of the pendulum and $\dot{\theta}$ is the angular velocity and continous-time dynamics:
\begin{align*}
dx = f(x, u)\:dt + C\:d\omega \qquad f(x,u) := \begin{bmatrix}
           \dot{\theta} \\
           a\sin \theta - b\:\dot{\theta} + u
         \end{bmatrix}    
\end{align*}
where $a>0$ summarizes the effects of gravity, mass and length of the pendulum, $b>0$ represents damping and friction, $u$ is the control input and $\omega$ is Brownian motion noise. The stage-cost at each state $x$ and control $u$ is:
\begin{align*}
g(x,u) = 1 - \exp(k\cos \theta-k) + \frac{r}{2}u^2           
\end{align*}
where $k>0$ determines the shape of the cost and $r>0$ scales the control cost. Note that the cost penalizes $x_1$ that is away from $0$ and is quadratic in the control $u$. Using Euler discretization with time step $\tau$ leads to the following discret-time dynamics:
\[
x_{k+1} = x_k + \tau f(x_k,u_k) + \epsilon_k, \quad \epsilon_k \sim \mathcal{N}(0,\tau CC^T)
\]
and discrete-time stage cost of $\tau g(x,u)$.



%============ Mountain Car ==============================%
\subsection{Mountain Car}
We consider a typical reinforcement learning benchmark problem known as the Mountain Car. A car is stuck between two mountains and its underpowered engine, even at full throttle, is unable to climb up the steep slope to the right (Fig.~\ref{fig:mountaincar}). The objective is to find a control policy that takes advantage of the potential energy obtained by swinging between the two mountains before driving straight towards the goal on the right. The state space is defined by the position $x$ of the car in the interval $[-1.2, 0.5] \: (m)$ and the velocity $v$ in $[-1.5, 1.5] \: (m/s)$. The height of the mountains is determined by $\sin(3x)$. There are three possible controls at each state $u \in \{-0.2, 0.0, 0.2\}$ representing the force applied to the car. The mass of the car is $m = 0.2\:kg$, the gravity is $g = 9.8\:m/s^2$, the friction is $k = 0.3$, and the time step is $\tau = 0.1s$. The terminal cost for reaching the goal is $-1$ and there is a stage cost of $0.01$ at each time step (we want to get there fast!). The discretized car dynamics are:
\begin{align*}
v_{t+1} &= v_t + \left(\frac{u_t}{m} -g\;m \cos(3x_t)  - k\;v_t\right) \tau\\
x_{t+1} &= x_t + v_{t+1} \tau.
\end{align*}
  


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/mountain_car.png}
  \caption{A car is stuck between two mountains and needs to find a way to overcome the steep slope to the right despite its underpowered engine.}
  \label{fig:mountaincar}
\end{figure}


%============ Cart-pole ==============================%
% http://www.matthewpeterkelly.com/tutorials/cartPole/
\subsection{Cart-pole}
The Cart-pole is another classical problem, considered a benchmark in reinforcement learning and control theory. The problem consists of a pole hinged on a cart which must be moved in order to keep the pole in vertical position. The state space consists of the position of the cart $x$, the velocity of the cart $\dot{x}$, the pendulum angle $\theta \in \left[-\frac{\pi}{2},\frac{\pi}{2}\right]$ rad (which is zero when the pole is perfectly vertical), and the pendulum angular velocity $\dot{\theta} \in [-\pi,\pi]$ rad/sec. The control input is the force $u \in [-50,50]$ Newton applied to the cart. The continuous time dynamics are~\cite{cartpole_dyn,cartpole_dyn_corr}:
\begin{align*}
\ddot{\theta} &= \frac{g \sin \theta - \cos \theta \brl{ \frac{u + m_2l\dot{\theta}^2\sin\theta}{m_1+m_2}}}{l \brl{\frac{4}{3} - \frac{m_2 \cos^2 \theta}{m_1+m_2}}}\\
\ddot{x} &= \frac{u + m_2 l \brl{\dot{\theta}^2 \sin\theta - \ddot{\theta} \cos \theta}}{m_1+m_2}
\end{align*}
The cart-pole dynamics discretized with time step $\tau$ are:
\begin{align*}
\theta_{t+1} &= \theta_t + \dot{\theta}_t \tau\\
\dot{\theta}_{t+1} &= \dot{\theta}_t + \frac{g \sin \theta_t - \alpha m_2 l (\dot{\theta}_t)^2 \sin(2 \theta_t)/2 + \alpha \cos(\theta_t) u_t}{4l/3 - \alpha m_2 l \cos^2(\theta_t)} \tau\\
x_{t+1} &= x_t + \dot{x}_t \tau\\
\dot{x}_{t+1} &= \dot{x}_t + \alpha\tau u_t + m_2 l \tau \dot{\theta}_t^2 \sin\theta_t - (\dot{\theta}_{t+1}-\dot{\theta}_t)\cos \theta_t
\end{align*}
where $m_1$ is the mass of the cart, $m_2$ is the mass of the pole, $l$ is the length of the pole, and $\alpha = 1/(m_1 + m_2)$. For example, $\tau = 0.1$ sec, $m_1 = 8$ kg, $m_2 = 2$ kg, $l = 0.5$ m, $g = 9.8\;m/s^2$.




%============ Acrobot ==============================%
\subsection{Acrobot}
We consider a deterministic double-pendulum system known as the acrobot (Fig.~\ref{?}). The acrobot state $x = \begin{pmatrix} \theta_1, \theta_2, \dot{\theta}_1, \dot{\theta}_2 \end{pmatrix}^T$ is defined by the joint angles $\theta_1$, $\theta_2$ and their velocities. The scalar control input $u$ is the torque acting on the second joint, leading to the following system dynamics:
\begin{align*}
\dot{x} &= a(x) + B(x)u\\
a(x) &= \begin{bmatrix} I_{2 \times 2} & 0\\ 0 & M^{-1}(x) \end{bmatrix} \begin{bmatrix} x_3 \\ x_4\\c_1(x)- \zeta x_3\\c_2(x)-\zeta x_4 \end{bmatrix}\\
B(x) &= \begin{bmatrix} I_{2 \times 2} & 0\\ 0 & M^{-1}(x) \end{bmatrix} \begin{bmatrix} 0\\0\\0\\1\end{bmatrix}\\
M(x) &= \begin{bmatrix} 3 + 2\cos(x_2) & 1+\cos(x_2)\\ 1+\cos(x_2) & 1 \end{bmatrix}\\
c_1(x) &= x_4(2x_3+x_4)\sin(x_2) + 2g\sin(x_1) + g\sin(x_1+x_2)\\
c_2(x) &= -x_3^2\sin(x_2) + g\sin(x_1+x_2)
\end{align*}
where $M(x)$ is the moment of inertia, $c_1(x)$, $(c_2(x))$ capture the coriolis, centripetal, and gravitational forces, $\zeta$ is the friction and $g$ is the gravity acceleration. The objective is to design a control policy which makes the acrobot stay in upright position $(\theta_1=\theta_2=0)$ with minimal control effort. Thus, we consider the stage cost:
\[
g(x,u) = 1 - e^{k \cos x_1 + k \cos x_2 - 2k} + \frac{r}{2} u^2
\]
where $r$ determines the relative importance of conserving control energy versus staying upright and $k$ is the width of the position cost.


